SniffySquad: Patchiness-Aware Gas Source Localization with Multi-Robot Collaboration

Gas source localization is pivotal for the rapid mitigation of gas leakage disasters, where mobile robots emerge as a promising solution. However, existing methods predominantly schedule robots' movements based on reactive stimuli or simplified gas plume models. These approaches typically excel in idealized, simulated environments but fall short in real-world gas environments characterized by their patchy distribution. In this work, we introduce SniffySquad, a multi-robot olfaction-based system designed to address the inherent patchiness in gas source localization. SniffySquad incorporates a patchiness-aware active sensing approach that enhances the quality of data collection and estimation. Moreover, it features an innovative collaborative role adaptation strategy to boost the efficiency of source-seeking endeavors. Extensive evaluations demonstrate that our system achieves an increase in the success rate by $20\%+$ and an improvement in path efficiency by $30\%+$, outperforming state-of-the-art gas source localization solutions.

==> design.tex <==

\section{Algorithm} \label{sec:design}

% \begin{figure*}[t]
%     \setlength{\abovecaptionskip}{0.2cm}
%     \setlength{\belowcaptionskip}{-0.3cm}
%     \centering
%     \includegraphics[width=1.95\columnwidth]{figs/overview.png}
%     \caption{System Architecture}
%     \label{fig:system_arch}
% \end{figure*}


% \begin{algorithm}[H]
% \caption{Weighted Tanimoto ELM.}\label{alg:alg1}
% \begin{algorithmic}
% \STATE 
% \STATE {\textsc{TRAIN}}$(\mathbf{X} \mathbf{T})$
% \STATE \hspace{0.5cm}$ \textbf{select randomly } W \subset \mathbf{X}  $
% \STATE \hspace{0.5cm}$ N_\mathbf{t} \gets | \{ i : \mathbf{t}_i = \mathbf{t} \} | $ \textbf{ for } $ \mathbf{t}= -1,+1 $
% \STATE \hspace{0.5cm}$ B_i \gets \sqrt{ \textsc{max}(N_{-1},N_{+1}) / N_{\mathbf{t}_i} } $ \textbf{ for } $ i = 1,...,N $
% \STATE \hspace{0.5cm}$ \hat{\mathbf{H}} \gets  B \cdot (\mathbf{X}^T\textbf{W})/( \mathbb{1}\mathbf{X} + \mathbb{1}\textbf{W} - \mathbf{X}^T\textbf{W} ) $
% \STATE \hspace{0.5cm}$ \beta \gets \left ( I/C + \hat{\mathbf{H}}^T\hat{\mathbf{H}} \right )^{-1}(\hat{\mathbf{H}}^T B\cdot \mathbf{T})  $
% \STATE \hspace{0.5cm}\textbf{return}  $\textbf{W},  \beta $
% \STATE 
% \STATE {\textsc{PREDICT}}$(\mathbf{X} )$
% \STATE \hspace{0.5cm}$ \mathbf{H} \gets  (\mathbf{X}^T\textbf{W} )/( \mathbb{1}\mathbf{X}  + \mathbb{1}\textbf{W}- \mathbf{X}^T\textbf{W}  ) $
% \STATE \hspace{0.5cm}\textbf{return}  $\textsc{sign}( \mathbf{H} \beta )$
% \end{algorithmic}
% \label{alg1}
% \end{algorithm}

\begin{algorithm}
    \caption{Replica Exchange Langevin Diffusion}\label{alg0}
    \begin{algorithmic}
        \WHILE{$Dist\_to\_Gas\_Source > Threshold$}
            \STATE $Env.\_Measurement \gets team\_sense()$
            \STATE $Global\_Map\_Probab.\_Est.(Env.\_Measurement)$
            \STATE $Team\_Navigation(Robots, Global\_Map)$
        \ENDWHILE
    \STATE
    \Function {Team\_Navigation}{$Robots, Global\_Map$}
            \FOR{$Robot\_A, Robot\_B\ in\ Robots$}
            \IF{$Check\_If\_Swap\_Roles(Robot\_A, Robot\_B)$}
            \STATE $Swap\_Roles(Robot\_A, Robot\_B)$ 
            \ENDIF
            \ENDFOR

            \FOR{$Robot\ in\ Robots$}
            \STATE $Grad \gets Calculate\_Gradient(Robot, Global\_Map)$
            \STATE $Pos_{t+1} \gets Set\_Goal\_LD(Robot, Global\_Map, Grad)$
            \STATE $Control(Robot)$
            \ENDFOR
    \EndFunction
    \end{algorithmic}
\end{algorithm}

\subsection{Probabilistic Gas Source Estimation} \label{subsec:estimation}
With the reframing of the GSL task as an optimization problem, the central focus lies in the definition of the potential function $\Phi(x)$ as stated in \cref{eq:min_Phi}. 
For every position $x\in \mathcal{X}$ in the environment, we estimate the probability that $x$ is located within the gas plume region. This probability estimation is denoted as $p(x)$, and subsequently, we define the potential function as: $\Phi(x) \doteq -log(p(x))$. 

To obtain $p(x)$ we employ a Bayesian estimation methodology, placing our method within the class of probabilistic GSL algorithms. Specifically, this estimator continually updates the likelihood of each position being situated within the gas plume region based on incoming measurements $z$ gathered from sensors equipped on the mobile robots. Mathematically, $p(x | z_{1:t}) \propto p(x | z_{1:t-1}) p(z_t | x,z_{1:t-1})$. 
In our scenario, the measurements $z=(z^c,z^w)\in \mathcal{Z}= \mathbb{R}\times \mathbb{R}^d$  collected from the mobile robots consists of the gas concentration $z^c$ and the wind vector $z^w$, acquired by chemical sensor and wind sensors (anemometers) respectively. 
To accommodate environments of arbitrary geometries, the area is discretized into a grid of equally-sized cells. 

The update procedure upon receiving new measurements is implemented based on \cite{ojeda2021information}, involving two sequential steps. 
(1) \textit{Local estimation generation}. 
% Let $U(x(t))$ denote the neighborhood region around the robot's current position $x(t)$. For positions $x \in U(x(t))$. The posterior probability of "the gas source being located at $x$" can be modeled using the wrapped normal distribution: \(p(x|z_{1:t}) = \frac{1}{\sigma \sqrt{2\pi}} \sum_{k=-\infty}^{\infty} \exp({-(\alpha(x,x(t))-\theta(z_t^w, z_t^c, x(t))+2\pi k)^2} / {2 \sigma^2})\). Here $\alpha:\mathcal{X}\times\mathcal{X} \to \Pi$ is the angle of the vector starting from $x(t)$ and pointing to position $x$. As for $\theta:\mathcal{Z} \times \mathcal{X} \to \Pi$, if $z_t^c \geq C$, it is the upwind direction; if $z_t^c < C$, $\theta(z_t^w, z_t^c) = \alpha(x(t), x(s))$ with $s$ satisfying $z_s^c \geq C$ and $\forall \tau \in (s,t], z_\tau^c <C$. 
The first step follows two intuitive and empirical rules: a) if the robot detects gas, the likelihood of neighboring grids within the upwind direction to localize within the gas plume is increased; b) If gas concentration is negligible or falls below a predefined threshold, grids directing to the position with previously recorded nonzero gas readings are attributed a higher likelihood of hosting gas. 
(2) \textit{Global estimation propagation}. 
The first step generates estimations solely for $x \in U(x(t))$, where $U(x(t))$ denotes the neighborhood region around the robot's current position $x(t)$, 
For the remaining areas $\{x \in \mathcal{X} \setminus U(x(t))\}$, their probabilities are updated in the second step by propagating information from $U(x(t))$ to the entire environment $\mathcal{X}$ based on \cite{ojeda2021information}, conforming to the geometry of the area. 


\subsection{recast}


\subsubsection{Problem reformulation}

% The gas source localization task using a team of $M$ robots aiming to reduce the search time $\mathcal{T}$ can be formulated as: 
% \begin{align} \label{eq:min_Phi}
%     \min_{\mathbf{u}\in \mathcal{U}^\mathcal{T}} & \mathcal{T}. \nonumber \\
%     \text{s.t.}     
%     & z_k = g(c_k, w_k) \nonumber \\
%     & b_{k+1} = h(b_k, z_k) \nonumber\\
%     & x^{(i)}_{k+1} = f(x^{(i)}_{k}, u^{(i)}_{k}) \nonumber
% \end{align} 
% where the time step is denoted as $k \in \mathcal{T}$. $z_k \in \mathcal{Z}$ is the local sensory measurements, $g: \mathbb{R} \times \mathbb{R}^d \to \mathcal{Z}$ is the observation model, $c_k$ and $w_k$ are values of the gas concentration and wind. $b_k \in \mathcal{B}$ is the belief of gas source's position, and $h: \mathcal{B} \times \mathcal{Z} \to \mathcal{B}$ is the estimator incorporating measurements to update $b_k$. $x^{(i)}_{k}$ is robot $i$'s position at time $k$, and $f: \mathcal{X} \times \mathcal{U} \to \mathcal{X}$ is the motion strategy that schedule the next waypoints based on positions of robot $i \in \{1, 2, \ldots, M\}$, other robots in the team $x^{(-i)}_{k}$, and the current belief. 

Our task, gas source localization, involves identifying a position with the highest probability of locating the source of a gas emission. In this context, we utilize a potential function denoted as $\Phi(x):\mathcal{X} \to \mathbb{R}$, which assesses the likelihood of position $x$ being the source location (position $x$ with a small value of $\Phi(x)$ has a high probability of being the source of gas leakage). Thus, the core task can be reinterpreted through an optimization lens, leading to the formulation: 
\begin{equation} \label{eq:min_Phi}
    \min_{x\in \mathcal{X}} \Phi(x). 
\end{equation} 
We describe the probabilistic estimator and the design of potential $\Phi(x)$ in \cref{subsec:estimation}. 

In the context of GSL, however, the optimization task presents notable challenges attributable to two factors.
First, the potential function exhibits multimodal characteristics and is far from convex due to the patchy gas plume. Second, the potential function available is noisy and stochastic \cite{kingma2014adam}. Specifically, the robots rely on measurements obtained from onboard sensors, which are susceptible to noise and provide partial observations. 
Consequently, conventional algorithms suitable for convex objectives and methods taking deterministic movements can be trapped and/or misled. 

\subsubsection{Optimization via sampling}
To deal with the challenges posed by the nonconvex and stochastic nature of the potential function, one promising approach is to reframe the optimization problem to an Markov chain Monte Carlo (MCMC) sampling problem \cite{cheng2020interplay}. 
% what is sampling? how to sampling a distribution? relationship between sampling and robot motion
Statistical sampling involves obtaining a sample of a desired probabilistic distribution. To this end, MCMC sampling methods first construct a Markov chain that has the desired distribution $\pi (x)$ as its equilibrium distribution, then one can obtain a sample of the intended distribution by recording states from the chain. Specifically, convergence to equilibrium means that the Markov chain 'forgets' about its initial state and the sequence of states after convergence subjects to distribution $\pi (x)$. 

\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.3cm}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/gashunter.png}
    \caption{System architecture}
    \label{fig:gashunter}
\end{figure}

% % Relationship between sampling and optimization
% Before clarifying the rationale behind embracing a sampling-based method, we illuminate the connections between optimization and sampling \cite{cheng2020interplay}. 
% In one direction, sampling algorithms can be viewed from an optimization perspective. By sampling a probability density function 
% \begin{equation} \label{eq:invariant_distribution}
%     \pi (x)=e^{- k \Phi(x)},
% \end{equation}
% random samples drawn from $\pi (x)$ will be attracted to the peak in the distribution $\pi (x)$, i.e., the global minimum of $\Phi(x)$. This relationship is exemplified when $\pi (x) = \delta(x^{*})$, where $x^{*} = \arg\min \Phi(x)$, as $k \rightarrow +\infty$. In particular, the Dirac delta equilibrium distribution concentrates at $x^{*}$ (the global minimum of $\Phi(x)$ and hence the position with the maximum likelihood of locating the source) and the chain 'forgets' about initial position of the mobile robot. 
% % why is the SDE called sampling ?
% Conversely, optimization algorithms can be expressed by a Markov chain for sampling. Stochastic gradient descent (SGD), for instance, $\Phi(x) = \frac{1}{\eta} \sum_{i=1}^{\eta} \Phi_{i} (x)$. It aligns with the form of a sampling procedure: $x \leftarrow x- \delta \nabla \Phi(x) + \delta \xi(x,\eta)$ where the noise term $\xi(x,\eta) = \nabla \Phi(x) - \frac{1}{\eta} \sum_{i=1}^{\eta} \Phi_{i} (x)$. 

% Advantages of MCMC sampling
As an alternative to optimization algorithms, Monte Carlo sampling algorithms have been shown to be powerful methods for nonconvex and multimodal optimization \cite{ma2019samplingcanbefaster, chen2020accelerating, deng2020contourSGLD} and noise and randomness in the potential function \cite{kingma2014adam}. 
Specifically, despite the fact that in the setting of convex functions, MCMC sampling is generally slower than optimization. For nonconvex objectives, however, sampling can be faster than optimization \cite{ma2019samplingcanbefaster}. 
Moreover, for noisy objectives whose randomness might arise from inherent function noise, MCMC sampling algorithms can be efficient by injecting the right amount of noise into each iterative update step, providing a means of coping with inherent noise. For instance, stochastic gradient descent methods \cite{kingma2014adam} are designed to cope with such randomness. 




\subsubsection{Langevin diffusion}\label{subsec:ld}

% diffusion process, SDE (discrete approximation, 
Diffusioin MCMC sampling methods simulates a Markov chain using diffusion processes, a concept from statistical physics describing the movement of particles. 
A diffusion process is defined by a stochastic differential equation (SDE), whose general form can be expressed as: 
\begin{equation}
    dx(t)= \mu(x(t)) dt+ \sigma(x(t)) dB(t), 
\end{equation}
where $x(t)$ is the positions of the particle. This SDE consists of a deterministic drift term $\mu(x(t))$ and a stochastic term, which is proportional to the standard Brownian motion $dB(t)$ and scaled by a factor $\sigma(x(t))$. 
The standard Brownian motion $\{B(t)\}_{t \geq 0}$ is a stochastic process with properties (i) movement during any time interval $(s,t) (s<t)$, $B(t-s) \doteq B(t)-B(s)$, is a normal random variable, i.e., $B(t-s) \sim \mathcal{N}(0,t-s)$, and (ii) the increments of different time intervals are independent.

% Langevin diffusion's SDE, intuitive description
The Langevin dynamic, with respect to the potential function $\Phi(x)$, is a diffusion process exhibits equilibrium behaviour. It is given by the stochastic differential equation: 
\begin{equation} \label{eq:langevin_diffusion}
    dx(t)=-\nabla \Phi(x(t)) dt+\sqrt{2 \tau} dB(t),
\end{equation} 
where $\nabla \Phi(x(t))$ is the gradient of the potential function at position $x(t)$, $\{B(t)\}_{t \geq 0}$ is a standard Brownian motion and $\tau > 0$ is a parameter called temperature in statistical physics and thermodynamics. 
Notably, \cref{eq:langevin_diffusion} is the stochastic version of gradient descent, differing in the incorporation of noise term, which is Gaussian with zero mean and a covariance determined by the temporal duration of the movement. 

% Langevin diffusion‘s equilibrium: Boltzmann distribution
This random process $\{x(t)\}_{t \geq 0}$ defined in \cref{eq:langevin_diffusion} has a unique invariant distribution (a.k.a. the Boltzmann-Gibbs distribution) with density 
\begin{equation} \label{eq:boltzmann_distribution}
    \pi_\tau (x)=\frac{e^{-\Phi(x)/\tau}}{\int_{\mathcal{X}} e^{-\Phi(x)/\tau} dx} = \frac{1}{Q} e^{-\Phi(x)/\tau}.
\end{equation}
Here the denominator $Q$ is the normalization constant. With any initial distribution of $x(t)$, the limiting distribution of $X_t$ converges to $\pi_\tau (x)$  by running the diffusion process. In other words, our solution is always expected to fall into the neighborhood of a global minimum of $\Phi(x)$ with high probability. 


% Combined with xxx, it can produce samples from. Compared to standard SGD, SGLD injects the right amount of Gaussian noise into the parameter updates to avoid collapses into local minima. 



% \subsection{Replica exchange}\label{subsec:re}

\subsubsection{Diffusion MCMC Sampling}
% temperature parameter
Langevin diffusion aids the escape from local minima by injecting noise into the gradient. However, the addition of perturbation may also encourage the agent to explore even if it is at the global optima, This gives rise to a balance between “global exploration” and “local exploitation", which correspond to high and low noise levels. This balance hinges on the temperature parameter $\tau$ in \cref{eq:boltzmann_distribution}. A high temperature fosters broader exploration across the global domain at the expense of reduced concentration around the minima, and vice versa. Therefore, the potential of using a fixed temperature is inherently limited.

% multiple temperatures
To attain the advantages of both behaviors and expedite convergence to global minima, techniques utilizing more than one temperature are employed. For example, simulated tempering \cite{marinari1992simulatedtempering} treats the temperature as a stochastic process. Rather than tracking only one diffusion process, another approach called parallel tempering (also known as replica exchange MCMC sampling) \cite{earl2005paralleltempering} tracks multiple diffusion processes driven by various temperatures and accelerates the convergence through swapping. 
% These techniques provide a way for accelerating the convergence of diffusion processes. In particular, when an agent is associated with a high temperature, it acts as the role of discovering new potential optima; when an agent has a low $\tau$, it focus on existing candidates of optima. 


\subsection{Patchy Plume-Resilient Movement Planning} \label{subsec:ld}

In this part, we describe the novel GSL motion strategy with resiliency to patchy gas plume caused by atmospheric turbulence and noisy partial observations from robots. 

We aim to develop a path planning strategy for source-seeking robots driven by Langevin dynamics. The Langevin diffusion is used to describe the motion of particles (or the update of parameters of machine learning models) by defining a continuous-time stochastic process. However, particle dynamics are different from the motion characteristics of mobile robots, hence they can not be directly applied. To establish a motion strategy suitable for robots, we first discretize the diffusion process and subsequently generate a sequence of positions for mobile robots to follow. 

In the first step, we attain a discrete-time algorithm through the Finite Difference Method. In detail, we first discretize the states over time from $\{x(t)\}_{t \in \mathbb{R}^{+}}$ to $\{x_k\}_{k \in \mathbb{Z}^{+}}$, where $x_k=x(k \cdot \delta t)$, and $\delta t$ represents the discretization time step size. Then we apply the explicit, forward-time Euler scheme for temporal discretization, leading to the following formulation of the discrete stochastic differential equation: 
\begin{equation} \label{eq:langevin_diffusion_discrete}
    x_{k+1} = x_{k} - \eta \cdot \nabla \Phi(x_k) + \sqrt{2 \eta \tau} \cdot \xi_{k}. 
\end{equation}
Here the stepsize $\eta > 0$ is proportional to the temporal discretization granularity $\delta t$, $\tau$ is the temperature parameter, and $\{\xi_k\}_{k\in \mathbb{Z}^+}$ signifies a sequence of standard normal random vectors. \cref{eq:langevin_diffusion_discrete} describes how the robot's motion evolves overtime while incorporating randomness. 

In the above equation, it requires calculating the gradient of the potential function at position $x$. However, the function we designed in \cref{subsec:estimation} is discrete and not differentiable. To address this, we adopt the central-difference approximation for spatial discretization: 
\[\nabla \Phi(x)\approx \begin{bmatrix} \frac{\Phi(x+h,y) - \Phi(x-h,y)}{2h}, & \frac{\Phi(x,y+h) - \Phi(x,y-h)}{2h} \end{bmatrix}^T.\] 
% $\nabla \Phi(x)\approx {[ (\Phi(x+h,y) - \Phi(x-h,y)) / 2h, (\Phi(x,y+h) - \Phi(x,y-h)) /2h ]}^T$.
Additionally, following gradients might force the robot jump between distant positions when the slope of the potential function at current position is substantial. For robots' path scheduling, we constrain the drift term to be below the robot's maximal velocity. 

\subsection{Collaborative Roles Adaptation} \label{subsec:re}    % for collaborative multi-robot GSL

In this part, we present how to coordinate a team of collaborative robots to balance the search efficiency and localization effectiveness by performing exploitation parsimoniously and executing exploration appropriately. This strategy consists of two tightly-coupled modules: \textit{Heterogeneous Roles Assignment} and \textit{Team Roles Adaptation}. 
% %role-based collaboration
% For the purpose of locating the gas source, we propose a multi-robot motion planning algorithm, consisting of division and adaptive exchange of robot roles, thereby empowering the system through tight collaboration and systematic coordination. 

\subsubsection{Heterogeneous Roles Assignment.} 
This module describes how robots in a team are assigned different roles to balance exploratory and exploitative plays. 

The scattered, patchy nature of gas plumes and the multimodal nature of concentration distribution map require an GSL system with two capabilities, (1) discovering new potential source positions and (2) distinguishing existing candidate positions. This gives rise to a trade-off between “global exploration” and “local exploitation" of the environment. To attain the advantages of both behaviors, we assign robots in the team with heterogeneous roles, named \textit{explorer} and \textit{exploiter} respectively. Robots acting as the former role are mainly responsible for objective (1) while the latter focus on objective (2). 

The role assignment can be implemented by regulating the temperature parameter in \cref{eq:langevin_diffusion}. Specifically, the temperature $\tau$ in the motion dynamic plays a crucial part in regulating the behaviour of the robot. Robots assigned a low temperature carry out exploitative actions while those with high temperatures engage in exploratory actions. 

Mathematically, for a team with $M$ robots, consider $M$ Markov chain driven by Langevin diffusions: 
\begin{equation} \label{eq:multi_langevin_diffusion}
    \mathrm{d}x^{(i)}(t)=-\nabla \Phi(x^{(i)}(t)) \mathrm{d}t+\sqrt{2 \tau^{(i)}(t)} \mathrm{d}B^{(i)}(t),
\end{equation}
where $i \in \{1, 2, \ldots, M\}$. The role of robot $i$ is specified by its temperature $\tau^{(i)}(t)$, which governs the extent of exploring potential gas source positions and exploiting local information to distinguish spurious gas patches. When a robot is assigned a low temperature, its motion is governed by the gradient of the potential function, the robot tends to exploit the local information of the surrounding potential field. For a robot with a higher temperature, more randomness is injected into the motion, it tends to explore the environment. 

The role division module, following \cref{eq:multi_langevin_diffusion}, is provided the guarantee that robots are expected to concentrate around the global minima of the potential function $\Phi(x)$. Specifically, we denote the positions of $M$ robots as $\mathbf{x} = \begin{bmatrix} x^{(1)}, x^{(2)}, \ldots, x^{(M)} \end{bmatrix}^T$, and their corresponding temperature parameters as $\mathbf{\tau} = \begin{bmatrix} \tau^{(1)}, \tau^{(2)}, \ldots, \tau^{(M)} \end{bmatrix}^T$. The invariant joint distribution \cite{chen2020accelerating} takes the form: 
\begin{equation} \label{eq:multi_boltzmann_distribution}
    \pi_{\mathbf{\tau}}(\mathbf{x}) \propto \exp\left( - \sum_{i=1}^{M} \frac{\Phi(x^{(i)})}{\tau^{(i)}} \right).
\end{equation}
The marginal stationary distribution of the low temperature robot will be attracted to the peak of the potential function $\Phi(x)$. 

\subsubsection{Team Roles Adaptation.} 
This submodule adaptively adjusts team roles through role swapping based on the principles of replica exchange. 

For optimizing trade-off between localization effectiveness and search efficiency, at an individual level, robots should exploit parsimoniously to avoid trapping in spurious patches and explore appropriately to escape from areas improbable to locate the source. From a team perspective, there should be some robots exploiting while others exploring. 

To adaptively optimize robot actions and systematically coordinate the team behavior, we propose a role-swapping mechanism for multi-robot GSL, incorporating replica exchange. When an exploiter $i$ locates at a position that is less likely to correspond to the desired gas source compared to an explorer $j$, this pair of robots swaps their roles. Consequently, robot $i$ transitions into an explorer so that it can turn to more promising areas and save time, while robot $j$ transforms into an exploiter who slows down and focuses to avoid missing the source of interest. 

Formally, this is achieved by swapping the temperatures between robots exhibiting different potential. Specifically, we consider a pair of random processes, denoted as robot $i$ and $j$, from the set of $M$ Langevin diffusions first. The two robots swaps temperatures with probability: 
\vspace{-0.20cm}
\begin{equation} \label{eq:re_swap_rate}
    s(i, j) = a \cdot \exp( \min(0, (\frac{1}{\tau^{(i)}}-\frac{1}{\tau^{(j)}}) \cdot (\Phi(x^{(i)})-\Phi(x^{(j)}))).
\end{equation}
Here the constant $a \geq 0$ represents the swapping intensity. 

In this manner, robots occupying positions associated with smaller potential function values are inclined to be assigned a role of exploiter, specified by a lower temperature, and vice versa. To elucidate the exchange rule, let us assume, without loss of generality, that $0 < \tau^{(i)} < \tau^{(j)} < \infty$ and $a = 1$. 
If $\Phi(x^{(i)}(t)) > \Phi(x^{(j)}(t))$, then robot $i$ swaps its temperature with robot $j$; otherwise, they swap with a probability $s(i, j) \in (0,1)$, which diminishes monotonically with respect to the difference between two objective values. For example, as $\Phi(x^{(i)}) \rightarrow 0$ and $\Phi(x^{(j)}) \rightarrow +\infty$, the swapping rate $s \rightarrow 0$. 

Under the specific swapping rule defined in \cref{eq:re_swap_rate}, the algorithm exhibits an acceleration effect in concentrating around the global minima of $\Phi(x)$. This effect is theoretically analysed and demonstrated in \cite{chen2020accelerating}. 
Meanwhile, sampling in this manner still leads to the minimization of potential function and hence the identification of the most probable gas source location. This is because the equilibrium distribution of the replica exchange Langevin diffusion is also \cref{eq:multi_boltzmann_distribution}, the same as algorithms in which robots follow independent diffusion processes in \cref{eq:multi_langevin_diffusion}. 

==> evaluation-bk.tex <==
\begin{figure*}[h]
    \setlength{\abovecaptionskip}{0.3cm}
    \setlength{\belowcaptionskip}{-0.0cm}
    \centering
    \includegraphics[width=2.0\columnwidth]{figs/scenario_final.png}
    \caption{Field experiment testbed of \textit{GasHunter}.}
    \label{fig:testbed}
\end{figure*}


\section{Performance Evaluation} \label{sec:eval}
In this section we evaluate the system's performance from two aspects: search effectiveness and search efficiency. We conduct extensive experiments to comprehensively evaluate the performance and advantages of \textit{GasHunter}. 
We first describe the settings of both physical and simulation experiments, as well as the metrics used in the evaluation (\S\ref{subsec:experiment_setting}). We then compare the overall performance of \textit{GasHunter} in both the testbed and simulation (\S\ref{subsec:eval_end2end}). We carry out experiments under different conditions to evaluate \textit{GasHunter}'s robustness to both external and internal factors (\S\ref{subsec:eval_robustness}). Finally, we perform an ablation study to further clarify each component (\S\ref{subsec:eval_ablation}). 




\begin{table}[!t]
% \setlength{\abovecaptionskip}{0.1cm}
% \setlength{\belowcaptionskip}{0.0cm}
    \caption{Configuration of Gas Dispersion Parameters}
    \label{tab:simulation_params}
    \centering
    \begin{tabular}{ccl}
        \toprule
        \textbf{Symbol} & \textbf{Value} & \textbf{Description} \\
        \midrule
        $\mu$  & $10 ppm$ & Gas conc. at filament center   \\
        $\sigma$ & $10 cm$ & Initial std of filament \\
        $\gamma$ & $10 cm^2/s$ & Growth ratio of $\sigma$  \\
        P, T              & 1 Atm, 298 Kelvins & Pressure and temperature  \\
        $\upsilon$ & $1.529\times 10^{-5} m^2/s$ & Kinematic viscosity \\
        $\rho$ & $1.196 kg/m^3$ & Air density \\
        $k$ & $3.75\times 10^{-3} m^2/s^2$ & Turb. kinetic energy \\
        $\varepsilon$ & $1.25\times 10^{-2} m^2/s^3$ & Dissipation rate \\
        \bottomrule
    \end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation and Setting} \label{subsec:experiment_setting}
% \textbf{Field Experiment Setup:} 
% We implement \textit{GasHunter} on a commercial unmanned ground vehicle. The robot is equipped with a particle matter sensor for concentration measurement, along with an ultrasonic anemometer for wind direction and speed sensing. 
% Generating gas plumes for conducting field experiments requires strictly safety and environmental considerations. As an alternative to this, a smoke machine that is commonly used on live stage performances was employed for controlled gas release. The primary component of the smoke fluid is ethylene glycol (EINECS No. 246-770-3). The behavior of such plumes mirrors that of numerous gas plumes in real-world application scenarios \cite{kadakia2022odour, francis2022gas}. 
% When ethylene glycol is atomized, it forms aerosol particles. We equip each robot with a particle sensor Plantower PMS5003T to measure the concentration of particles with diameters below 3 micrometers, denoted in units of $\mu g/m^3$. 
% An industrial fan was utilized to generate the turbulent wind field. 
% We conducted tests on a rectangular field measuring $15m \times 10m$ in an enclosed laboratory environment.
% To determine the ground truth positions of the robots and source, a UWB localization device is integrated. To drive the robots to the desired positions, a PID controller is utilized. 
% For the collaborative estimation and search strategy, the onboard computer of our mobile olfactory robot is a Raspberry Pi 4 Computer Model B with 8GB RAM, and the server is equipped with Intel(R) Core(TM) i7-11700 of 2.50GHz main frequency and 16G RAM, running the Ubuntu 20.04.4 operating system. 
% space size
% fog machine and PMS
% fan and windsonic
% UWB localization
% central server

\subsubsection{Field Experiment Setup}
\textbf{Gas Environment}:
We build a gas leakage testbed in a rectangular $15m \times 10m$ laboratory environment with turbulent wind from outside, as shown in Fig. \ref{fig:testbed}.
Generating gas plumes for conducting field experiments requires strict safety and environmental considerations. 
Therefore, we simulate the gas leakage scenario by adopting a smoke machine as the gas generator to release gas following previous work \cite{bourne2019coordinated, hutchinson2019experimental, hutchinson2018information}. The primary component of the smoke fluid is ethylene glycol (EINECS No. 246-770-3). The behavior of such plumes mirrors that of numerous gas plumes in real-world application scenarios \cite{kadakia2022odour, francis2022gas}. 
\textbf{Multi-robot platform}: 
We implement \textit{GasHunter} on commercial unmanned ground vehicles. Each robot is equipped with a particle matter sensor for concentration measurement, along with an ultrasonic anemometer for wind direction and speed sensing. When ethylene glycol is atomized, it forms aerosol particles. We equip each robot with a particle sensor Plantower PMS5003T to measure the concentration of particles with diameters below 3 micrometers, denoted in units of $\mu g/m^3$. 
To establish ground truth positions, a UWB localization device is integrated. Robot movement is guided by a PID controller. 
For the collaborative estimation and search strategy, the onboard computer of our mobile olfactory robot is a Raspberry Pi 4 Computer Model B with 8GB RAM, and the server is equipped with Intel(R) Core(TM) i7-11700 of 2.50GHz main frequency and 16G RAM, running the Ubuntu 20.04.4 operating system. 

\begin{figure*}[t]
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.3cm}
\centering
    \subfigure[Success Rate]{
        \centering
        \includegraphics[width=0.66\columnwidth]{figs/numrobot_successrate.png}
        %\caption{fig1}
        \label{fig:numrobot_successrate}
    }%
    \subfigure[Search Time]{
        \centering
        \includegraphics[width=0.66\columnwidth]{figs/numrobot_searchtime.png}
        \label{fig:numrobot_searchtime}
    }%
    \subfigure[Path Efficiency]{
        \centering
        \includegraphics[width=0.66\columnwidth]{figs/numrobot_pathefficiency.png}
        \label{fig:numrobot_pathefficiency}
    }%
% \caption{Overall performance of \textit{GasHunter} and related works evaluated using different metrics.}
\caption{Overall performance of physical feature-based simulation experiments.}
\label{fig:overall_metrics}
\end{figure*}

% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.0cm}
% \setlength{\belowcaptionskip}{-0.3cm}
% \centering
%     \subfigure[Path Efficiency]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/field_numrobot_pathefficiency.png}
%         \label{fig:field_numrobot_pathefficiency}
%     }%
%     \subfigure[Search Time]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/field_numrobot_searchtime.png}
%         \label{fig:field_numrobot_searchtime}
%     }%
% \caption{Field experiment results.}
% \label{fig:field_numrobot}
% \end{figure}

% \textbf{Simulation Setting:} 
\subsubsection{Simulation Setting}
% The data used for simulation is generated using two tools: (i) OpenFOAM \cite{jasak2009openfoam}, a computational fluid dynamics (CFD) simulator, is used to generate the wind flow vector field; (ii) GADEN \cite{monroy2017gaden}, a 3-D gas dispersion simulator widely recognized and commonly used for robotic olfaction, is used to generate the gas concenrtation field. Specifically, the data generation process involves the following two steps. First, OpenFOAM models the flow of wind based on the environment geometry that is configured by a computer-aided design (CAD) model, and the specified flow inlets and outlets. Second, based on the wind flow data, GADEN takes the environment CAD model as input and obtains 3D gas distributions by implementing the filament gas dispersion theory \cite{farrell2002filament}. In our experiments, the data is generated based on materials provided in \cite{ojeda2021information} and our parameter configuration is listed in \cref{tab:simulation_params}. 
% The geometry of environment used in simulation includes two representative scenarios in industrial factories: (i) empty spaces and (ii) environments with rooms featuring walls and obstacles. 
We build up the simulation environment based on two tools: (i) OpenFOAM \cite{jasak2009openfoam}, a computational fluid dynamics (CFD) simulator, is used to generate the wind flow vector field; (ii) GADEN \cite{monroy2017gaden}, a 3-D gas dispersion simulator widely recognized and commonly used for robotic olfaction, is used to generate the gas concentration field. Specifically, the data generation process involves the following two steps. First, OpenFOAM models the flow of wind based on the environment geometry that is configured by a computer-aided design (CAD) model, and the specified flow inlets and outlets. Second, based on the wind flow data, GADEN takes the environment CAD model as input and obtains 3D gas distributions by implementing the filament gas dispersion theory \cite{farrell2002filament}. In our experiments, the data is generated based on materials provided in \cite{ojeda2021information} and our parameter configuration is listed in \cref{tab:simulation_params}. 
The geometry of environment used in simulation includes two representative scenarios in industrial factories: (i) empty spaces and (ii) environments with rooms featuring walls and obstacles. 



% \begin{table}[htbp]
%     \centering
%     \small % Set font size to small
%     \begin{tabular}{cc}
%     \toprule
%     \textbf{Important Configuration} & \textbf{Value} \\
%     \midrule
%     filament\_initial\_std  & 10 \\
%     filament\_initial\_std  & 10 \\
%     filament\_growth\_gamma & 10 \\
%     filament\_noise\_std    & 10 \\
%     gas\_type               & 10 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Simulation Configuration}
%     \label{tab:simulation_params}
% \end{table}

% \documentclass{article}



% \textbf{Comparative Methods:} 
\subsubsection{Comparative Methods}
We compared \textit{GasHunter} with two state-of-the-art strategies in mobile robot olfaction (MRO)-based gas source localization to extensively evaluate the performance of \textit{GasHunter}: 
1) \textbf{Surge-Cast} \cite{reddy2022olfactory}, a SOTA bio-inspired GSL algorithm. It's a reactive algorithm inspired by the movement patterns of male moths navigating within windy and turbulent plumes. The operational strategy involves two distinct motions: when the robot identifies the plume concentration exceeding a predefined threshold, it engages in a "surge", i.e., moving upwind; otherwise, it executes a "cast" maneuver perpendicular to the wind direction to re-establish contact with the plume. 
2) \textbf{Infotaxis} \cite{vergassola2007infotaxis,ojeda2021information}, a SOTA probabilistic GSL algorithm. It's an information-driven path planning algorithm, leveraging a probability map of the source position estimation and driving the robot's movement toward the place with the highest information gain.  



% \subsection{Evaluation Metrics} \label{subsec:eval_metrics}
% \textbf{Evaluation Metrics:}
\subsubsection{Evaluation Metrics}
An ideal gas source localization algorithm is expected to achieve two key objectives: (i) Effectively localizing the source position; (ii) Efficiently searching the source in an unknown area, thereby saving time during gas source localization. 
To comprehensively assess \textit{GasHunter}'s performance in relation to these goals, we evaluate the algorithms employing the following three metrics: 

\noindent (1) \textbf{Success Rate}. It is determined by calculating the ratio of successful trails across all repeated experiments. A trial is deemed successful if mobile olfactory robots reach the vicinity of the actual ground truth position of the gas source within the predefined time limit and distance threshold. In practical application scenarios, the gas leakage source can be detected using onboard cameras as soon as it comes within a robot's line-of-sight. 

\noindent (2) \textbf{Search Time}. In the case of successful trials, the search time is defined as the time from the moment of departure to the instance of arrival at the source position. 

\noindent (3) \textbf{Path Efficiency}. The generated trajectories' Efficiency is defined as $d_{min} / d$, where $d_{min}$ is the shortest path distance from the robot's starting point to the gas source, $d$ is the length of the robot's travel trajectory driven by GSL approaches. This metric is also only calculated for successful trials. 
 
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.3cm}
\centering
    \subfigure[Search Time]{
        \centering
        \includegraphics[width=0.48\columnwidth]{figs/field_numrobot_searchtime.png}
        \label{fig:field_numrobot_searchtime}
    }%
    \subfigure[Path Efficiency]{
        \centering
        \includegraphics[width=0.48\columnwidth]{figs/field_numrobot_pathefficiency.png}
        \label{fig:field_numrobot_pathefficiency}
    }%
% \caption{Field experiment results.}
\caption{Overall performance of \textit{GasHunter}.}
\label{fig:field_numrobot}
\end{figure}

\subsection{End-to-end System Evaluation} \label{subsec:eval_end2end}


\begin{figure*}[t]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.1cm}
\centering
    \includegraphics[width=1.9\columnwidth]{figs/traj-B.jpg}
\caption{In an empty space (w/o walls and obstacles). (a)-(c) Illustration of trajectories generated by Surge-Cast, Infotaxis, and \textit{GasHunter}. (d) The distance of the robot to the gas release source over time. }
\label{fig:overall_illustration-B}
\end{figure*}


\begin{figure*}[t]
% \setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
% \setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
% \setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subcaption
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.1cm}
\centering
    \includegraphics[width=1.9\columnwidth]{figs/traj-C.jpg}
\caption{In a structured space (w/ walls and obstacles). (a)-(c) Illustration of trajectories generated by Surge-Cast, Infotaxis, and \textit{GasHunter}. (d) The distance of the robot to the gas release source over time. }
\label{fig:overall_illustration-C}
\end{figure*}

% \subsubsection{Physical experiments.}
The overall performance evaluated in the testbed is shown in \cref{fig:field_numrobot}. 
In terms of both path efficiency and search time, the performance of \textit{GasHunter} surpasses two SOTA baselines, Surge-Cast and Infotaxis. \textit{GasHunter} improves the path efficiency (i.e., decreases the trajectory lengths) by $32\%$ and $32\%$ compared to Surge-Cast and Infotaxis, respectively; and it reduces search time by $67.5 s$ and $14 s$, respectively. 
We also compare the results between field experiments and physical-feature-based simulation, and both sets of results exhibit similar results among the three methods. Specifically, \textit{GasHunter} improves the path efficiency by $39\%$ and $28\%$ and reduces search time by $20.6\%$ and $15.2\%$, respectively. This similarity verifies that \textit{GasHunter}, which aims to improve the search efficiency by explicitly considering the patchiness of the gas plumes in real world, brings significant benefits to mobile robot olfaction-based gas source localization. 

% \subsubsection{Simulation experiments.}

The overall performance of \textit{GasHunter} is further evaluated extensively by simulation in two representative scenarios in industrial factories: (i) an open space (measuring $100m$ by $60m$) and (ii) an area with the existence of walls, rooms and obstacles ($100m$ by $100m$). We compare the performance of \textit{GasHunter} as well as two state-of-the-art algorithms, Surge-Cast and Infotaxis. 

\cref{fig:overall_metrics} quantifies the efficacy of \textit{GasHunter} under different metrics for GSL, using both an individual robot and a team of robots. These experiments were carried out 50 times for each configuration. 
For all algorithms, the success rate shows an upward trend as the number of robots employed for gas source search and localization increases. 
Across all scenarios involving robot counts ranging from one to three, it is evident that \textit{GasHunter} consistently attains the highest success rate, achieves the shortest search time for both an individual robot and robot teams, and generates the most efficient path. Specifically, \textit{GasHunter} achieves a success rate of 76\% for a team of three robots, improving by $30\%$ and $20\%$ in comparison with Surge-Cast and Infotaxis, respectively. The search time and path efficiency is $148 s$ and $0.67$, reducing the total search time by $22.92\%$ and $18.46\%$, shortening the trajectory length by $41.79\%$ (from $2.56 d_{min}$ to $1.49 d_{min}$) and $32.84\%$ (from $2.22 d_{min}$ to $1.49 d_{min}$), respectively. 


\cref{fig:overall_illustration-B} and \cref{fig:overall_illustration-C} further illustrate the performance of these methods. 
In \cref{fig:overall_illustration-B} (a)-(c) and \cref{fig:overall_illustration-C} (a)-(c), it is demonstrated that \textit{GasHunter} produces smoother trajectories than baselines. Surge-Cast, a reactive method relying solely on current observations to make decisions, yields inefficient zig-zag paths and is the most susceptible to spatial and temporal gas concentration fluctuations (as shown in \cref{fig:conc_distr_characteristic}). Infotaxis, though incorporating a Bayesian gas source position estimator to filter the sensory measurements, suffers from trap in patchy areas. 
In \cref{fig:overall_illustration-B} (d) and \cref{fig:overall_illustration-C} (d), it's verified that \textit{GasHunter} navigates towards the source the most efficiently and arrives at the source the most quickly. In the empty space scenario, Surge-Cast takes $231$ seconds and Infotaxis takes $187$ seconds in total while \textit{GasHunter} takes only $145$ seconds, indicating a decrease in search time by $37.23\%$ and $22.46\%$ in comparison to the two baselines, respectively. In the environment with walls and rooms, the three methods take $371$, $339$, and $299$ seconds respectively, i.e., \textit{GasHunter} reduces the search time by $19.40\%$ and $11.80\%$. The acceleration effect produced by \textit{GasHunter} relative to previous methods in localizing the source attributes to the movement planning method that regulates the robots' moving direction to enable escaping from gas patches, as well as the collaborative assignment and adaptation of team roles. 




% With the growth in the number of robots within the team, our method exhibits an augmented success rate. However, this increase in success rate corresponds to an elongation of search time and a minor decline in path efficiency. A balance must be struck between success rate and search time, where a higher temperature setting translates to an elevated success rate but longer trajectory lengths. A higher temperature setting would make the robot's exploration strategy more aggressive, leaning towards exploration rather than exploitation. Consequently, the robot would explore more diverse areas before reaching the source, resulting in longer search distances. Even though there's a trade-off between path efficiency and a higher success rate, our proposed method outperforms all other baseline strategies in terms of search time and path efficiency. For SurgeCast, robots operate independently, and there is no significant observable impact on performance with varying numbers of robots. 


\subsection{System Robustness} \label{subsec:eval_robustness}
% \subsection{Impact of External Factors}
% Factors that are out of the direct control of XX may influence its performance,


% In this context, the gas release rate, wind speed and temperature in the algorithm are all taken into consideration as they are the three factors we believe exert the most significant influence on the search process. 
% When the gas release rate is low, it results in a more patchy gas plume, as elaborated in section x, which in turn escalates the complexity of the search process. 
% On the other hand, the magnitude of the wind field dictates diverse combinations of gas distribution and patchiness levels. 
% Moreover, from an algorithmic perspective, the temperature parameter directly dictates the style of search, whether it leans more towards exploration or exploitation. A higher temperature leads to a more aggressive search strategy, aiming to comprehensively explore the map as extensively as possible. 
% Thus, we have investigated the impact of these three factors on the proposed method to demonstrate its superiority. 


\begin{figure*}
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{-0.3cm}
    \begin{minipage}[b]{0.9\columnwidth}
    \centering
        \subfigure[Weak source]{
            \centering
            \includegraphics[width=0.46\columnwidth]{figs/Qheatmap.png}
            %\caption{fig1}
            \label{fig:Q_illustration-weak}
        }%
        % \subfigure[Q=30]{
        %     \centering
        %     \includegraphics[width=0.31\columnwidth]{figs/Qheatmap-20.png}
        %     \label{fig:Q_illustration-moderate}
        % }%
        \subfigure[Strong source]{
            \centering
            \includegraphics[width=0.46\columnwidth]{figs/Qheatmap-30.png}
            \label{fig:Q_illustration-strong}
        }%
    \caption{Snapshots of gas concentration field under different emission intensity. }
    \label{fig:Q_illustration}
    \end{minipage}
    \begin{minipage}[b]{1.1\columnwidth}
    \centering
        \subfigure[Success Rate]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/Q_successrate.png}
            %\caption{fig1}
            \label{Q_successrate}
        }%
        % \subfigure[Search Time]{
        %     \centering
        %     \includegraphics[width=0.66\columnwidth]{figs/Q_mst.png}
        %     \label{Q_mst}
        % }%
        \subfigure[Path Efficiency]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/Q_pathefficiency.png}
            \label{Q_pathefficiency}
        }%
    \caption{Impact of gas emission intensity.} % our approach is especially good at scenario of the weak source (more patchy)
    \label{fig:Q_metrics}
    \end{minipage}
\end{figure*}

\begin{figure*}
    \begin{minipage}[h]{1.3\columnwidth}
        \subfigure[Success Rate]{
            \centering
            \includegraphics[width=0.48\columnwidth]{figs/geometry_successrate.png}
            %\caption{fig1}
            \label{fig:geometry_successrate}
        }%
        \subfigure[Path efficiency]{
            \centering
            \includegraphics[width=0.48\columnwidth]{figs/geometry_pathefficiency.png}
            \label{fig:geometry_pathefficiency}
        }%
    \setlength{\abovecaptionskip}{0.0cm}
    \setlength{\belowcaptionskip}{-0.3cm}
    \caption{\textbf{Impact of the env. geometry.}}
    \label{fig:geometry}
    \end{minipage}\hfill
    \begin{minipage}[h]{0.7\columnwidth}
        \centering
        \vspace{0.5cm}
        \includegraphics[width=1.0\columnwidth]{figs/D0_searchtime_pathefficiency.png}
        \caption{Impact of $D_0$ (initial distance to source).}
         % The nearer the robots places initially, The higher the Success rate and the shorter the search time. 
        \label{fig:D0}
    \end{minipage}
\end{figure*}


\subsubsection{Gas Emission Intensity.} 
We verify the robustness of the system in scenarios with different release rate of the gas source. First, we clarify the relationship between the weak source and patchy gas plume, as depicted in \cref{fig:Q_illustration}. Second, we demonstrate in \cref{fig:Q_metrics} that \textit{GasHunter} outperforms the baselines especially under the weak gas source, where the difficulty posed by the patchy nature of the plume is exacerbated. 

\textit{Weak Gas Source \& Patchy Gas Plume.} 
The gas emission intensity influences characteristics of the gas concentration field. As shown in \cref{fig:Q_illustration}, a weaker gas emission source leads to more patchy gas plumes, consequently increasing the difficulty of gas source localizaion. 

We divide the gas emission intensity into two categories, weak and strong, corresponding to the demands of different GSL applications. In \cref{fig:Q_illustration-weak}, the weak source indicates a slow gas filament release rate with $Q=10$ per second, while in \cref{fig:Q_illustration-strong} the strong source represents a quick release rate with $Q=30$ per second, respectively. 


\cref{fig:Q_metrics} shows the results of success rate and path efficiency of motion strategies under the weak and strong gas source. 
% From the obtained results, it is evident that our proposed method demonstrates remarkable robustness against fluctuations in the gas source release rate. Across weak, moderate, and strong gas source scenarios, our method consistently achieves the highest success rate, the shortest search time, and the most efficient paths among all the approaches. 
Firstly, for all the three methods, the performance degrades from the strong source to weak source scenario. Surge-Cast, Infotaxis, and our approach's path efficiency decreases (trajectory length increase) from $2.56 d_{min}$, $2.22 d_{min}$, and $1.64 d_{min}$ to $1.82 d_{min}$, $1.67 d_{min}$, and $1.45 d_{min}$, respectively. The success rate of Surge-Cast and Infotaxis decreases from $0.52$ and $0.7$ to $0.46$ and $0.56$ on average. 
Secondly, across scenarios of the strong and weak source, \textit{GasHunter} consistently achieves the highest success rate and the most efficient paths among all methods. 
The success rate is increased by $0.38$ and $0.28$ from Surge-Cast and Infotaxis to our method in the weak source scenario, increased by $0.32$ and $0.14$ in the strong source scenario. Meanwhile, the path efficiency is increased by $0.36$ and $0.26$ from Surge-Cast and Infotaxis to \textit{GasHunter} in the weak source, increased by $0.20$ and $0.13$ in the strong source. 

It's noteworthy that our approach's advantages is especially significant under the weak gas source, validating its remarkable robustness to gas emission intensity. From the strong to weak source scenario, Surge-Cast and Infotaxis's success rates decrease considerably by $12\%$ and $20\%$, respectively, their trajectory lengths increases (path efficiency decreases) largely by $41\%$ and $33\%$, respectively. In contrast, our method's success rate does not decreases and its path efficiency slightly reduces by only $13\%$. 
The performance of baselines are susceptible to the weak emission intensity, as the efficacy of localizing the source deteriorates drastically; on the other hand, our method eliminates the degradation effect of patchy gas plumes, which is particularly a significant issue under the weak source of leakage. This can be attributed to the mechanism to escape from spurious gas patches and the role-based collaboration algorithm. 


\begin{figure*}[t]
    \setlength{\abovecaptionskip}{0.0cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \subfigure[Individual Robot]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/tau_1robot_successrate_pathefficiency.png}
            \label{fig:tau_1robot}
        }%
        \subfigure[Multiple Robot]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/tau_2robot_ho_successrate_pathefficiency.png}
            \label{fig:tau_homo}
        }%
        \caption{Impact of temperature parameter.}
        \label{fig:tau}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \subfigure[Patchy-resilient Movement Planning]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/tau_2robot_wVSo_LD.png}
            \label{fig:wVSo_LD}
        }%
        \subfigure[Collaborative Role Adaptation]{
            \centering
            \includegraphics[width=0.5\columnwidth]{figs/tau_2robot_hoVShe_successrate_pathefficiency.png}
            \label{fig:hoVShe}
        }%
        \caption{Ablation study}
        \label{fig:ablation}
    \end{minipage}
\end{figure*}


\subsubsection{Geometry of the Environment.}
We evaluate the robustness of our approach in different environment geometries. As show in \cref{fig:geometry}, we evaluate GSL methods in an empty space (without obstacles) and structured environment (with walls and rooms), and verify the consistent benefits of our method. The average success rates are $84\%$ and $70\%$ in empty and structured scenes, respectively, which increase $28\%$ and $20\%$ compared to the best results of two baselines. The path efficiency are $1.64 d_{min}$ and $1.59 d_{min}$, reducing the search path length by $26.2\%$ and $33.3\%$, respectively, compared to the best results of baselines.



% \subsubsection{Impact of the number of robots.}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.70\columnwidth]{figs/M_searchtime_pathefficiency.png}
%     \caption{Impact of the M (number of robots). as M increases, success rate increases and path efficiency decreases}
%     \label{fig:tau_1robot}
% \end{figure}


\subsubsection{Initial Distance to the Source $D_0$}
We examine the impact of robots' initial distances to the gas source on the task. The robots initiate their journey from five distinct positions, ranging from close to gradually increasing distances relative to the gas source. The results are shown in \cref{fig:D0}. As seen, the difficulty of source-seeking within predeterminied time limit gradually grows with increasing distance, and the success rate are $1.0$, $1.0$, and $0.7$ for the distances of $50m$, $70m$, and $90m$, respectively. When the initial distance rises to over $70m$, the ratio of success trials decreases and the search time increases. Nevertheless, \textit{GasHunter} can still achieve the gas source localization in $148.1s$ in average when the robots are at least $90m$ away from the source at departure. 



\subsubsection{Temperature Parameters}
As clarified in \cref{sec:algo2}, the temperature $\tau$ is a critical parameter in the system as it governs the role of a robot. We conduct experiments to evaluate the impact of the temperature values on the performance of our system. We analyze the impact of $\tau$ on both an individual and multiple robots' behavior in \cref{fig:tau}. 

% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.0cm}
% \setlength{\belowcaptionskip}{-0.4cm}
% \centering
%     \subfigure[Individual Robot]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/tau_1robot_successrate_pathefficiency.png}
%         %\caption{fig1}
%         \label{fig:tau_1robot}
%     }%
%     \subfigure[Multiple Robot]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/tau_2robot_ho_successrate_pathefficiency.png}
%         \label{fig:tau_homo}
%     }%
    
% \caption{Impact of Temperature Parameter.}
% \label{fig:tau}
% \end{figure}




\textit{Individual Robot.} 
We evaluate the impact of a single robot's temperature on the performance of localizing the gas source. To this end, we examine the temperature values $\tau$ across five orders of magnitude. As illustrated in \cref{fig:tau_1robot}, the results of success rate and path efficiency exhibits a different trend as the temperature rises. 
Firstly, the results indicate an increase and subsequent decrease in success rate with rising temperature. With a moderate temperature, the success rate on average is $0.8$; on the other hand, with an extremely low or high temperature the success rate decreases to $0.4$ and $0.3$ when $\tau=10^{-3}$ and $\tau=10^1$, respectively. Secondly, the path efficiency diminishes as the temperature increases, especially when it rises over $\tau=10^{-1}$. The trajectory lengths increases by merely $1.2\%$ from $\tau=10^{-3}$ to $\tau=10^{-1}$, but increases by $9\%$ from $\tau=10^{-1}$ to $\tau=10^0$. 
This pattern emerges because, a robot exploits or explores excessively fails to both search efficiently and localize the source effectively. Specifically, associating with an exceeding low or high temperature, the robots' motion focus locally or explores globally without combining both behaviors' advantages. 

\textit{Multiple Robots.} % with Homogeneous Temperatures 
\cref{fig:tau_homo} shows the effect of the temperature parameters $\{\tau_i \mid i = 1,2,\cdots,M\}$ on the system's performance, measured by success rate, search time, and path efficiency. To clarify the impact with respect to values of $\tau$, robots in the team are assigned a same temperature. 
For multiple robots, the performance outcomes resemble those of the single robot case as shown in \cref{fig:tau_1robot}, given that the roles of the three robots are identical. 
% ... numerical declarations ...



\subsection{Ablation Study} \label{subsec:eval_ablation}
We further conduct an ablation study to understand the effectiveness of components introduced in \cref{sec:algo1,sec:algo2}. 

% \begin{figure}
% \setlength{\abovecaptionskip}{0.0cm}
% \setlength{\belowcaptionskip}{-0.3cm}
%     \centering
%     \subfigure[Motion Strategy]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/tau_2robot_wVSo_LD.png}
%         %\caption{fig1}
%         \label{fig:wVSo_LD}
%     }%
%     \subfigure[ERA2]{
%         \centering
%         \includegraphics[width=0.48\columnwidth]{figs/tau_2robot_hoVShe_successrate_pathefficiency.png}
%         \label{fig:hoVShe}
%     }%
%     \caption{Ablation Study}
%     \label{fig:ablation}
% \end{figure}

\subsubsection{Effectiveness of the Patchy Plume-Resilient Movement Planning.}
In this experiment, we compare the gas source localization performance without (w/o) and with (w/) the proposed Patchy Plume-Resilient Movement Planning component to show the performance gains it brings into the overall system. The results are shown in \cref{fig:wVSo_LD}. As seen,  with our movement planning algorithm, the system achieves an enhanced performance, where the success rate increases without sacrificing the path efficiency and search time. Specifically, the success rate of success rate of \textit{GasHunter} with the novel motion strategy is $0.9$, increasing that of \textit{GasHunter} without the motion strategy by $\sim 30\%$. Meanwhile, the trajectory lengths and total search time is increased by merely $4.3\%$ and $1.4\%$, respectively. 

\subsubsection{Effectiveness of the Collaborative Roles Adaptation strategy.}
To demonstrate the effectiveness of the Collaborative Role Adaptation module in the \textit{GasHunter}, we evaluate the localization effectiveness and search efficiency with and without assigning different roles and adaptively adjusting them through \cref{eq:re_swap_rate}. The results are shown in \cref{fig:hoVShe}. We divide the teams of robots into two categories, homogeneous and heterogeneous, where robots are acting the same role and different roles, respectively. Specifically, heterogeneous teams consist of all combinations in which at least one robot acts a different role from others, and the metrics are averaged for experiments using a range of temperature values. The success rate, trajectory length (path efficiency), and search time improves $0.64$, $1.49 d_{min}$, and $142 s$ to $0.7$, $1.43 d_{min}$, and $136 s$, respectively. 
The approach without the Role Assignment and Adjustment module is surpassed by the approach with the component, utilizing the complementary capabilities of multiple robots and further exploits them through adaptive role swapping. Specifically, this is attributed to the distinct temperatures representing diverse roles within the team, which forms the basis of the role exchange mechanism in the proposed method. This underscores that flexible allocation of roles within a team enhances agile exploration or exploitation of robots, effectively expediting global-scale search while mitigating local optima concerns. 

==> introduction-20240112.tex <==
\section{Introduction}


\IEEEPARstart{L}{ocalizing} the gas leak source rapidly is of paramount importance. 
Unforeseen gas leaks can swiftly create a highly flammable atmosphere, which will lead to risks of explosions, health hazards, as well as long-term environmental impacts, especially when the gas is toxic \cite{liu2017individualized, pal2018vehicle, maag2018w}. For instance, the Bhopal gas tragedy exposed over 500,000 people to methyl isocyanate (MIC) \cite{mishra2009bhopal}, while the Aliso Canyon blowout released over 100,000 tonnes of greenhouse gas methane into the atmosphere \cite{conley2016methane}. 
It is crucial to note that only after locating the source can subsequent mitigation measures, such as shutting off valves and effectively containing or sealing the leaks, be executed \cite{liu2017delay}.


Nonetheless, gas source localization (GSL) in emergent scenarios has not been effectively resolved \cite{motlagh2023unmanned, abughanam2023localization}. 
Specifically, extensive and complex pipelines offer numerous potential points of leakage, rendering it impractical to install sensors at every juncture \cite{ojeda2020evaluation}. 
Furthermore, assigning human operators to engage in these laborious and perilous activities not only introduces the risk of human error in interpretation \cite{arain2021sniffing}, but also poses a risk to their health and lives \cite{ojeda2023robotic}.

\begin{figure}[t]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    % \includegraphics[width=0.6\columnwidth]{figs/scenario.jpeg}
    % \includegraphics[width=0.3\columnwidth]{figs/Qheatmap.png}
    \includegraphics[width=0.98\columnwidth]{figs/fig1.png}
    
    \caption{Mobile olfactory robots autonomously search for and navigate towards the source of gas leakage. }
    \label{fig:scenario}
\end{figure}

% As an alternative, the deployment of autonomous mobile olfactory robots offers a viable solution for gas source localization. This approach is attractive not only for its safety but also its efficiency \cite{arain2021sniffing}. As illustrated in \cref{fig:scenario}, in the event of a gas leakage within a factory's pipeline system, a fleet of robots equipped with gas concentration sensors can be dispatched to search for and locate the source of the leakage. 

Deploying autonomous mobile olfactory robots for GSL presents a solution with great potential \cite{iyer2019living, moradi2018skycore, khochare2021heuristic}, as they can search the environment with high efficiency without risking human lives \cite{xu2022swarmmap, zhou2022swarm}. 
We task gas leakage in a factory with intricate pipelines as an example as shown in \cref{fig:scenario}. Here, a fleet of robots equipped with gas concentration sensors and wind sensors are dispatched to search the surroundings and gather gas sensory data. By analyzing and interpreting the environmental conditions, the robots autonomously navigate to pinpoint the source of the gas leak.
% This is nontrivial for two reasons. 
% First, as illustrated in \cref{fig:conc_distr_characteristic}, the turbulent airflow in real-world scenarios \cite{kadakia2022odour} causes the gas plume to fragment and become significantly patchy \cite{reddy2022olfactory}. Second, the mobile robots can only access to noisy sensory measurements and partial observations, unable to get an accurate and global understanding of the field. 
% Consequently, inferring the source position from robots' measurements becomes intractable \cite{ojeda2023robotic}. 

% Unfortunately, current approaches are not able to offer feasible solutions for autonomous mobile robot olfaction-based gas source localization in realistic environments, which typically resort to two broad categories of strategies:
Existing GSL solutions can be roughly grouped into two categories: 
(1) Reactive bio-inspired algorithms. 
These solutions draw inspiration from the behavior of insects or rodents. They involve moving up the local gas concentration gradients (chemotaxis), responding to air currents and moving upwind (anemotaxis), or combining both \cite{reddy2022olfactory}. 
(2) Source parameter estimation-based GSL. 
These solutions estimate the source location utilizing the Bayesian filter, making decisions based on historical data. 

\IEEEpubidadjcol

However, these methods either work only in ideal continuous concentration fields or heavily rely on oversimplified and unrealistic analytical gas plume models, such as the Gaussian plume model\cite{vergassola2007infotaxis, bourne2019CoordinatedBayesianBasedBioinspired, bourne2020decentralized}. 
In reality, the gas landscape is typically discontinuous and characterized by a \textit{patchy} structure, where the gas forms distinct and scattered areas, as shown in \cref{fig:conc_distr_characteristic}(b).
Therefore, these models deviate significantly from the complexity of patchy gas distribution in real-world scenarios. 
% As shown in \cref{fig:conc_distr_characteristic} (a), these models deviate significantly from the complexity of patchy gas distribution in real-world scenarios. 
% \begin{figure}[!t]
%     \setlength{\abovecaptionskip}{0.2cm}
%     \setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figs/fig2.png}
%     \caption{Spatial characteristics of the gas concentration distribution.}
%     \label{fig:conc_distr_characteristic}
% \end{figure}
\begin{figure}[!t]
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/fig2-20240314.png}
    \caption{Real-world spatial characteristics of gas concentration distribution are observed within a sub-area of our testbed. A gas emission device is positioned on the left side, and winds blow from left to right. The heatmap illustrates Concentration values, representing the number of particles with a diameter $>$0.3um in 0.1L of air. The gas plume patches may mislead source seeking robots into incorrectly identifying these (false positives) as the actual source of the gas emission. }
    \label{fig:conc_distr_characteristic}
\end{figure}

\textbf{Our work} aims to enhance collaborative mobile robots olfactory sensing with resiliency to \textit{patchy} gas plumes in realistic atmospheric environments. 
% Furthermore, we find significant drawbacks when attempting to deploy previous solutions in real-world environments. 
This problem is non-trivial due to the following two challenges:

% Challenge 1: Turbulence, patchy, intermittent
% \noindent $\bullet$ \textbf{The patchy nature of gas plumes confuses and traps robots in gas patches}. 
% Numerous patches create multiple modes (i.e., hills) in the concentration field, causing robots utilizing noisy and local information (e.g., gradient) on such a map to confuse and get stuck in local optima. Additionally, in regions between patches, the robot might have trouble discerning the correct direction to move in due to low or zero gas concentration readings, which make the robot uncertain about whether it is moving towards or away from the source. 
\noindent $\bullet$ \textbf{The patchy nature of gas plumes confuses and traps the robots locally (C1)}. 
% Numerous patches create multiple modes (i.e., hills) in the concentration field, causing robots utilizing noisy and local information (e.g., gradient) on such a map to confuse and get stuck in local optima. Additionally, in regions between patches, the robot might have trouble discerning the correct direction to move in due to low or zero gas concentration readings, which make the robot uncertain about whether it is moving towards or away from the source. 
% As demonstrated by experimental data in Fig. \ref{fig:conc_distr_characteristic}(b), plumes fragment into disjointed patches spatially. The gas concentration measured along the horizontal centerline (\cref{fig:conc_distr_characteristic}(c)) exhibits pronounced fluctuations as the distance to the source increases, which indicates the patches are separated by regions where gas concentration is below detection. This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches.
As demonstrated by experimental data in Fig. \ref{fig:conc_distr_characteristic}, plumes fragment into disjointed patches spatially. The gas concentration measured along the horizontal centerline exhibits pronounced fluctuations as the distance to the source increases, which indicates the patches are separated by regions where gas concentration is below detection \cite{rigolli2022alternation}. This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches \cite{reddy2022olfactory}.



% Challenge 2
\noindent $\bullet$ \textbf{A patchy plume demands an efficient global search, conflicting with the goal of effective gas source localization for collaborative robots (C2)}. 
The robot team conducting GSL strives to (i) identify new potential gas source positions and (ii) exclude false potential source positions. These two goals are inconsistent and render it hard to schedule multiple robots collaboratively \cite{biswas2023mode, jing2021recent}. Specifically, for the former goal, the robots are required to disperse and explore disjoint areas independently. Conversely, the latter goal demands the robots to converge to the same location to confirm source probability through multiple measurements.


In this paper, we propose \textit{GasHunter}, a collaborative multi-robot olfaction-based system for gas source localization. It conquers the patchy characteristic of gas plumes and enables efficient and effective source localization via cooperation, as elaborated below.
To address the first challenge (\textbf{C1}) and achieve individual-level resiliency, we propose a novel \textit{Patchy Plume-Resilient Movement Planning} method. 
This is achieved by adjusting the robots' gradient-based moving direction with a regulation term. This term injects the motion with an appropriate amount of perturbation, enabling them to escape from false positive source positions efficiently.
To address the second challenge (\textbf{C2}) and achieve team-level resiliency, we devise a \textit{Potential-instructed Collaborative Roles Adaptation} strategy for multiple robots to balance the search efficiency and localization effectiveness. 
% 1
Robots in the team collaboratively estimate the potential of each position locating the emission source. 
% 2
Those positioned in areas with higher probabilities conduct fine-grained search to inspect spurious concentration maxima (\textit{exploiter}), while other robots perform coarse-grained search to discover new potential sources (\textit{explorer}). 
% Robots are assigned heterogeneous roles that represent different planning preferences. For example, some robots are responsible for inspecting spurious concentration maxima (\textit{exploiter}), while others are in charge of discovering new potential source positions (\textit{explorer}). 
% 3
When an explorer finds potential sources with higher probability than an exploiter, they exchange roles, so that the explorer becomes an exploiter while the exploiter is released for course-grained search. 
In this manner, the robots' roles are adjusted adaptively based on their current positions and the potential to localize the source in the surroundings, thus parallelizing the exploration of the environment and exploitation of collected information in a flexible manner.

% In contrast, existing methods tailored for cooperative GSL either rely on gathering or scattering, so they lack efficiency in achieving both goals. In Particle Swarm Optimization (PSO)-based algorithms \cite{duisterhof2021sniffy}, robots follow the one who discovers a better pattern (potential source), resulting in gathering behavior \cite{chen2019odor}. On the contrary, another approach \cite{bourne2019CoordinatedBayesianBasedBioinspired} dispatches robots to investigate several likely source positions separately, inducing scattering behavior. 

% To the best of our knowledge, we are the first to handle the turbulent airflow and patchy gas plume issue from the view of nonconvex learning. 
We validate our design with experiments on a multi-robot testbed in a $15m \times 10m$ space and large scale physical feature based simulations in two different scenarios. Experiment results show that our system achieves $20\%+$ success rate improvement and $30\%+$ path efficiency improvement compared to state-of-the-art methods~\cite{reddy2022olfactory,ojeda2021information,vergassola2007infotaxis}.
% We implemented the proposed system on an indoor gas emission testbed, in a  $15m \times 10m$ space. We build a team of olfactory unmanned ground vehicles to conduct the gas source localization task. 
% We further conduct comprehensive simulation experiments with various number of robots in two different scenarios (an empty space and a structured environment). 
% We compare our system with the state-of-the-art (SOTA) of both bio-inspired and probabilistic GSL algorithms, Surge-Cast \cite{reddy2022olfactory} and Infotaxis \cite{ojeda2021information,vergassola2007infotaxis}. The experiment results show that our system achieves success rates higher than baselines by $> 20\%$, outperforming then in path efficiency by $> 32.84\%$. 
% We then examine the robustness of our system under various conditions and finally conduct an ablations study to understand each module in our system. 
We summarize the contributions of this paper as follows:
% \begin{itemize}
% \item A patchy plume-resilient movement strategy that navigates across patchy gas plumes. 
% \item A heterogeneous team roles assignment and adaptation algorithm that balances search efficiency (global exploration) and localization effectiveness (local exploitation) by role-swapping, incorporating replica exchange. 
% \item Validation and evaluation in both a testbed and a physical-feature-based gas dispersion simulator rooted in the principles of Computational Fluid Dynamics. 
% \end{itemize}
\begin{itemize}
\item We design \textit{GasHunter}, a collaborative multi-robot olfactory sensing system for gas source localization, specifically designed to handle the patchy characteristic in realistic gas plume environments.
\item We devise a patchy plume-resilient movement strategy inspired by non-convex learning to conquer the complex patchy characteristic of gas plumes.
\item We develop a collaborative strategy for multiple robots by assigning and adapting their planning preferences dynamically to balance the search efficiency and localization effectiveness of gas sources.
\item Extensive experiments are conducted for validation and evaluation in both a real-world testbed and a physical-feature-based gas dispersion simulator. 
\end{itemize}

The remainder of the paper is organized as follows. We first introduce the background, motivation, and related works in \cref{sec:background}. In \cref{sec:systemmodel}, we present the overview and components of our system model, followed by problem formulation. In \cref{sec:algo1,sec:algo2}, we introduce the algorithm design, involving detailed descriptions of the patchy plume-resilient movement planning and collaborative roles adaptation. \cref{sec:eval} showcases the implementation and evaluation. Finally, \cref{sec:conclusion} concludes the paper. 

==> introduction-20240314.tex <==
\section{Introduction}


\IEEEPARstart{L}{ocalizing} the gas leak source rapidly is of paramount importance. 
Unforeseen gas leaks can swiftly create a highly flammable atmosphere, which will lead to risks of explosions, health hazards, as well as long-term environmental impacts, especially when the gas is toxic \cite{liu2017individualized, pal2018vehicle, maag2018w}. For instance, the Bhopal gas tragedy exposed over 500,000 people to methyl isocyanate (MIC) \cite{mishra2009bhopal}, while the Aliso Canyon blowout released over 100,000 tonnes of greenhouse gas methane into the atmosphere \cite{conley2016methane}. 
It is crucial to note that only after locating the source can subsequent mitigation measures, such as shutting off valves and effectively containing or sealing the leaks, be executed \cite{liu2017delay}.


Nonetheless, gas source localization (GSL) in emergent scenarios, like those mentioned above, has not been effectively resolved \cite{motlagh2023unmanned, abughanam2023localization}. 
Specifically, extensive and complex pipelines offer numerous potential points of leakage, rendering it impractical to install sensors at every juncture \cite{ojeda2020evaluation}. 
Furthermore, assigning human operators to engage in these laborious and perilous activities not only increases the risk of misinterpretation \cite{arain2021sniffing}, but also poses a risk to their health and lives \cite{ojeda2023robotic}.

\begin{figure}[t]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    % \includegraphics[width=0.6\columnwidth]{figs/scenario.jpeg}
    % \includegraphics[width=0.3\columnwidth]{figs/Qheatmap.png}
    \includegraphics[width=0.98\columnwidth]{figs/fig1.png}
    
    \caption{Mobile olfactory robots autonomously search for and navigate towards the source of gas leakage. }
    \label{fig:scenario}
\end{figure}

% As an alternative, the deployment of autonomous mobile olfactory robots offers a viable solution for gas source localization. This approach is attractive not only for its safety but also its efficiency \cite{arain2021sniffing}. As illustrated in \cref{fig:scenario}, in the event of a gas leakage within a factory's pipeline system, a fleet of robots equipped with gas concentration sensors can be dispatched to search for and locate the source of the leakage. 

Deploying autonomous mobile olfactory robots for GSL presents a solution with great potential \cite{iyer2019living, moradi2018skycore, khochare2021heuristic}, as they can search the environment with high efficiency without risking human lives \cite{xu2022swarmmap, zhou2022swarm}. 
We take gas leakage in a factory with intricate pipelines as an example as shown in \cref{fig:scenario}. Here, a fleet of robots equipped with gas concentration sensors and wind sensors are dispatched to search the surroundings and gather gas sensory data. By analyzing and interpreting the environmental conditions, the robots autonomously navigate to pinpoint the source of the gas leak.
% This is nontrivial for two reasons. 
% First, as illustrated in \cref{fig:conc_distr_characteristic}, the turbulent airflow in real-world scenarios \cite{kadakia2022odour} causes the gas plume to fragment and become significantly patchy \cite{reddy2022olfactory}. Second, the mobile robots can only access to noisy sensory measurements and partial observations, unable to get an accurate and global understanding of the field. 
% Consequently, inferring the source position from robots' measurements becomes intractable \cite{ojeda2023robotic}. 

% Unfortunately, current approaches are not able to offer feasible solutions for autonomous mobile robot olfaction-based gas source localization in realistic environments, which typically resort to two broad categories of strategies:
Existing olfactory robot-based GSL solutions can be roughly grouped into two categories: 
(1) Reactive bio-inspired algorithms. 
These solutions draw inspiration from the behavior of insects or rodents. They involve moving up the local gas concentration gradients (chemotaxis \cite{benichou2011intermittent}), responding to air currents and moving upwind (anemotaxis \cite{rahbar20173}), or combining both \cite{reddy2022olfactory}. 
(2) Source parameter estimation-based GSL. These solutions estimate the source location utilizing the Bayesian filter, making decisions based on historical data. 
However, these methods either work only in ideal continuous concentration fields or heavily rely on oversimplified and unrealistic analytical gas plume models, such as the Gaussian plume model\cite{vergassola2007infotaxis, bourne2019CoordinatedBayesianBasedBioinspired, bourne2020decentralized}. 
Such models exhibit substantial deviation from the complex gas distribution in practical environments.
\IEEEpubidadjcol

In reality, the gas landscape is characterized by a \textit{patchy} structure, which renders the aim to enhance the practicability of GSL non-trivial. Specifically, as demonstrated by field measurements of concentration (\cref{fig:conc_distr_characteristic}), the gas plumes in realistic atmospheric environments fragment into disjointed patches and form distinct and scattered areas. 
From the perspective of source seeking robots, the concentration measured along the horizontal centerline exhibits pronounced fluctuations as the distance to the source increases \cite{rigolli2022alternation}, since gas patches are separated by regions where gas concentration is below detection. This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches \cite{reddy2022olfactory}.



% \begin{figure}[!t]
%     \setlength{\abovecaptionskip}{0.2cm}
%     \setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figs/fig2.png}
%     \caption{Spatial characteristics of the gas concentration distribution.}
%     \label{fig:conc_distr_characteristic}
% \end{figure}
\begin{figure}[!t]
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/fig2-20240314-220ppi.png}
    % \caption{Real-world spatial characteristics of gas concentration distribution are observed within a sub-area of our testbed. A gas emission device is positioned on the left side, and winds blow from left to right. The heatmap illustrates concentration values, representing the number of particles with a diameter $>$0.3um in 0.1L of air. The gas plume patches may mislead source seeking robots into incorrectly identifying these (false positives) as the actual source of the gas emission. }
    \caption{\rev{\textbf{Spatial characteristics of gas concentration}. We conducted a proof-of-concept experiment to check gas characteristics in our indoor testbed, with a gas emission device at $(1.0,1.0)$ and winds blowing along the $x$ axis. The heatmap illustrates concentration values, representing the number of particles with a diameter $>$0.3um in 0.1L of air. The observed gas plume patches may mislead source-seeking robots into falsely identifying them as the actual gas emission source.}} 
    \label{fig:conc_distr_characteristic}
\end{figure}


% % C2
% In terms of system implementation, another challenge rises. A patchy plume demands an efficient global search, conflicting with the goal of effective gas source localization for collaborative robots. 
% The robot team conducting GSL strives to (i) identify new potential gas source positions and (ii) exclude false potential source positions. These two goals are inconsistent and render it hard to schedule multiple robots collaboratively \cite{biswas2023mode, jing2021recent}. Specifically, for the former goal, the robots are required to disperse and explore disjoint areas independently. Conversely, the latter goal demands the robots to converge to the same location to confirm source probability through multiple measurements.


To tackle the above challenge, we propose \textit{GasHunter}, a collaborative robotic olfactory system towards practical gas source localization. The design and implementation of \textit{GasHunter} boosts adaptability to patchiness at both the individual and the team level, making \textit{GasHunter} achieve more efficient and effective emission source localization. For each individual, we devise individual active sensing algorithms aimed at improving the quality of estimation; for the whole team, we develop collaborative roles adaptation strategies to enhance the efficiency of source seeking. Overall, our method features the following two key designs: 

% To achieve individual-level resiliency, we propose a \textit{Patchiness-aware Active Sensing} method. It improves the collected data effectiveness (the quality of sampled data) by movement coordination. This is achieved by adjusting the robots' gradient-based moving direction with a regulation term. This term injects the motion with an appropriate amount of perturbation, enabling them to escape from false positive source positions efficiently.
\noindent $\bullet$ At the individual level, we propose a \textit{Patchiness-aware Active Sensing} method, which builds on probabilistic source estimation and embeds principles of Langevin MCMC, to improve the quality of collected data and estimation. % (integrates deterministic and stochastic components of sensing direction)
This is achieved by incorporating a regulatory term into the robots' gradient-based sensing direction. This enables escape from false positive source positions, resulting in the collection of more valid and informative data.

% To implement a system with team-level resiliency, we devise a \textit{Potential-instructed Collaborative Roles Adaptation} strategy for multiple robots. It enhances source-seeking efficiency and accelerate the GSL process. 
\noindent $\bullet$ At the team level, we devise a \textit{Potential-instructed Collaborative Roles Adaptation} strategy, which leverages both external environmental cues and internal team dynamics, to enhance source-seeking efficiency and accelerate the GSL process. 
Specifically, robots in the team collaboratively estimate the potential of each position locating the emission source. 
Those positioned in areas with higher probabilities conduct fine-grained search to inspect spurious concentration maxima (exploiter), while other robots perform coarse-grained search to discover new potential sources (explorer). 
When an explorer finds potential sources with higher probability than an exploiter, they exchange their roles to allow flexible collaboration. %, so that the explorer becomes an exploiter while the exploiter is released for course-grained search. 
% In this manner, the robots' roles are adjusted adaptively based on their current positions and the potential to localize the source in the surroundings, thus parallelizing the exploration of the environment and exploitation of collected information in a flexible manner.



% To the best of our knowledge, we are the first to handle the turbulent airflow and patchy gas plume issue from the view of nonconvex learning. 
We validate our design with experiments on a multi-robot testbed in a $15m \times 10m$ space and large scale physical feature based simulations in two different scenarios. Experiment results show that our system achieves a $20\%+$ success rate improvement and a $30\%+$ path efficiency improvement compared to state-of-the-art methods~\cite{reddy2022olfactory,ojeda2021information,vergassola2007infotaxis}.
% We implemented the proposed system on an indoor gas emission testbed, in a  $15m \times 10m$ space. We build a team of olfactory unmanned ground vehicles to conduct the gas source localization task. 
% We further conduct comprehensive simulation experiments with various number of robots in two different scenarios (an empty space and a structured environment). 
% We compare our system with the state-of-the-art (SOTA) of both bio-inspired and probabilistic GSL algorithms, Surge-Cast \cite{reddy2022olfactory} and Infotaxis \cite{ojeda2021information,vergassola2007infotaxis}. The experiment results show that our system achieves success rates higher than baselines by $> 20\%$, outperforming then in path efficiency by $> 32.84\%$. 
% We then examine the robustness of our system under various conditions and finally conduct an ablations study to understand each module in our system. 
We summarize the contributions of this paper as follows:
% \begin{itemize}
% \item A patchy plume-resilient movement strategy that navigates across patchy gas plumes. 
% \item A heterogeneous team roles assignment and adaptation algorithm that balances search efficiency (global exploration) and localization effectiveness (local exploitation) by role-swapping, incorporating replica exchange. 
% \item Validation and evaluation in both a testbed and a physical-feature-based gas dispersion simulator rooted in the principles of Computational Fluid Dynamics. 
% \end{itemize}
\begin{itemize}
\item We design \textit{GasHunter}, a collaborative multi-robot olfactory sensing system for gas source localization, specifically designed to handle the patchy characteristic in realistic gas plume environments.
\item We devise a patchiness-aware active sensing method, which builds on probability source estimation and embeds principles of Langevin dynamics, to improve the quality of collected data and estimation.
\item We develop a potential-instructed collaborative roles adaptation strategy, which leverages both external environmental cues and internal team dynamics, to enhance source-seeking efficiency and accelerate the GSL process. 
\item Extensive experiments are conducted for validation and evaluation in both a real-world testbed and a physical-feature-based gas dispersion simulator. 
\end{itemize}

The remainder of the paper is organized as follows. We first introduce the background, motivation, and related works in \cref{sec:background}. In \cref{sec:systemmodel}, we present the overview and components of our system model, followed by problem formulation. In \cref{sec:algo1,sec:algo2}, we introduce the algorithm design, involving detailed descriptions of the patchiness-aware active sensing and potential-instructed collaborative roles adaptation. \cref{sec:eval} showcases the implementation and evaluation. Finally, \cref{sec:conclusion} concludes the paper. 

==> introduction-20240928.tex <==
\section{Introduction}


% \IEEEPARstart{L}{ocalizing} the gas leak source rapidly is of paramount importance. 
% Unforeseen gas leaks can swiftly create a highly flammable atmosphere, which will lead to risks of explosions, health hazards, as well as long-term environmental impacts, especially when the gas is toxic \cite{liu2017individualized, pal2018vehicle, maag2018w}. For instance, the Bhopal gas tragedy exposed over 500,000 people to methyl isocyanate (MIC) \cite{mishra2009bhopal}, while the Aliso Canyon blowout released over 100,000 tonnes of greenhouse gas methane into the atmosphere \cite{conley2016methane}. 
% It is crucial to note that only after locating the source can subsequent mitigation measures, such as shutting off valves and effectively containing or sealing the leaks, be executed \cite{liu2017delay}.


Rapid and accurate responses to gas leak incidents are essential for safeguarding human and environmental health, as leaked gases can rapidly create highly flammable or toxic conditions, posing significant risks of explosions and poisoning. For instance, in the United States alone, 2,600 gas leakage incidents were reported, with 328 resulting in explosions and 122 fatalities~\cite{sun2024gastag}. A key aspect of quick response involves localizing the gas source, which involves analyzing the concentration and distribution of the gas in the air to trace it back to its origin. With the knowledge of source locations, subsequent mitigation operations, such as shutting off valves or sealing the leaks, can be conducted more logically, efficiently, and safely. 


% Nonetheless, gas source localization (GSL) in emergent scenarios, like those mentioned above, has not been effectively resolved \cite{motlagh2023unmanned, abughanam2023localization}. 
% Specifically, extensive and complex pipelines offer numerous potential points of leakage, rendering it impractical to install sensors at every juncture \cite{ojeda2020evaluation}. 
% Furthermore, assigning human operators to engage in these laborious and perilous activities not only increases the risk of misinterpretation \cite{arain2021sniffing}, but also poses a risk to their health and lives \cite{ojeda2023robotic}.

Conventional gas source localization (GSL) solutions fall into two categories: 
($i$) human expert-based solutions assign human operator to engage in affected areas. These laborious and perilous activities not only increase the risk of misinterpretation but also endanger the lives of the operators~\cite{mccarron2018air};
($ii$) wireless sensor network (WSN)-based methods utilize preinstalled static sensors to detect the gas source by monitoring gas concentration readings~\cite{manes2016realtime}. This techniques suffer from spatial resolution limitations, especially when extensive and complex pipelines exist and provide numerous potential points of leakage. 

% Deploying autonomous mobile olfactory robots for GSL presents a solution with great potential \cite{iyer2019living, moradi2018skycore, khochare2021heuristic}, as they can search the environment with high efficiency without risking human lives \cite{xu2022swarmmap, zhou2022swarm}. 
% We take gas leakage in a factory with intricate pipelines as an example as shown in \cref{fig:scenario}. Here, a fleet of robots equipped with gas concentration sensors and wind sensors are dispatched to search the surroundings and gather gas sensory data. By analyzing and interpreting the environmental conditions, the robots autonomously navigate to pinpoint the source of the gas leak.

Fortunately, deploying multiple mobile olfactory robots presents a promising solution, as the robots can search the environment with high efficiency without risking human lives. We take gas leakage scenario in a factory with intricate pipelines as an example, as shown in \cref{fig:scenario}. Here, a fleet of robots equipped with gas concentration sensors and wind sensors are dispatched to search the surroundings and gather gas sensory data. By analyzing and interpreting the environmental conditions, the robots autonomously navigate to pinpoint the source of the gas leakage.


\begin{figure}[t]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    % \includegraphics[width=0.6\columnwidth]{figs/scenario.jpeg}
    % \includegraphics[width=0.3\columnwidth]{figs/Qheatmap.png}
    \includegraphics[width=0.98\columnwidth]{figs/fig1.png}
    
    \caption{Mobile olfactory robots autonomously search for and navigate towards the source of gas leakage. }
    \label{fig:scenario}
\end{figure}



% Existing olfactory robot-based GSL solutions can be roughly grouped into two categories: 
% (1) Reactive bio-inspired algorithms. 
% These solutions draw inspiration from the behavior of insects or rodents. They involve moving up the local gas concentration gradients (chemotaxis \cite{benichou2011intermittent}), responding to air currents and moving upwind (anemotaxis \cite{rahbar20173}), or combining both \cite{reddy2022olfactory}. 
% (2) Source parameter estimation-based GSL. These solutions estimate the source location utilizing the Bayesian filter, making decisions based on historical data. 
% However, these methods either work only in ideal continuous concentration fields or heavily rely on oversimplified and unrealistic analytical gas plume models, such as the Gaussian plume model\cite{vergassola2007infotaxis, bourne2019CoordinatedBayesianBasedBioinspired, bourne2020decentralized}. 
% Such models exhibit substantial deviation from the complex gas distribution in practical environments.
% \IEEEpubidadjcol


By fully embracing the new advantages brought by autonomous robots, recent innovations explore the scheduling of multi-robots for enhancing GSL in challenging scenarios, which can be roughly grouped into two types: 
($i$) \textit{bio-inspired algorithms} leverage local gas concentration gradients or airflow directions detected by each robot to guide their movements toward potential source locations. While effective in simple scenarios, they often fail in complex real-world situations where local gradient does not necessarily lead to the source. % characterized by turbulent airflow.
($ii$) \textit{probabilistic model-based approaches} estimate the source locations based on analytical gas dispersion models and incoming measurements from all robots. These methods heavily rely on oversimplified and unrealistic gas dispersion models. % , limiting their effectiveness to ideal scenarios with continuous concentration gas fields. 

% \noindent ($i$) \textit{model free/bio-inspired algorithms} leverage local gas concentration gradients or airflow directions detected by each robot to guide their movements toward potential source locations. While effective in simple scenarios, they often fail in complex real-world situations characterized by turbulent airflow.

% \noindent ($ii$) \textit{model-based approaches} estimate the source locations based on prior knowledge of gas dispersion models and incoming measurements from all robots. These methods, while more robust, heavily rely on oversimplified and unrealistic gas dispersion models, limiting their effectiveness to ideal scenarios with continuous concentration gas fields. 
% \com{describe the disadv. of their cooperation style}

In summary, both types of methods exhibit limited effectiveness in realistic scenarios with patchy gas concentration fields. This brings about the first challenge we focus on:
\textbf{ (C1) The patchy nature of gas plumes confuses and traps the robots.}
% \noindent $\bullet$ \textbf{ (C1) The patchy nature of gas plumes confuses and traps the robots.}
In reality, the gas landscape is characterized by a \textit{patchy} structure. As demonstrated by field measurements of gas concentration (see \cref{fig:conc_distr_characteristic}), gas plumes in realistic atmospheric environments fragment into disjointed patches and form distinct and scattered areas. 
From the perspective of source seeking robots, the concentration measured along the horizontal centerline exhibits pronounced fluctuations as the distance to the source increases, since gas patches are separated by regions where gas concentration is below detection. 
This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches and failure to complete GSL.

From the perspective of system implementation, we face a second challenge:
\textbf{(C2) Trade-off between source localization effectiveness and search efficiency for collaborative robots.}
% \noindent $\bullet$ \textbf{The patchy nature of gas plumes confuses and traps the robots.}
Since gas distribution varies continuously over space and time, it is impossible to measure at every possible location all the time. Therefore, the robot strives to (\textit{i}) identify new potential gas source positions and (\textit{ii}) exclude false potential source positions, with a limited number of samples. These two goals are inconsistent and render it hard to localize the true source position with both effectiveness and efficiency. Specifically, for the former goal, the robot is required to explore the area and sample the gas information. Conversely, the latter goal demands the robots to exploit previously acquired information to reach the estimated source localization and confirm its probability. Existing multi-robot GSL solutions lead to either gathering or scattering collaborative behaviors, highlighting the potential for further enhancement in collaboration. 

\noindent \textbf{Remark}. As far as we are aware, previous works develop their operating principles ignoring the patchy nature of gas plumes, based on which they schedule each agent identically without fully harnessing robots' collaborative capabilities at a system level.  


\noindent \textbf{Our work}. We aim to devise an effective strategy for collaboratively scheduling multiple olfactory robots to localize the gas source in real-world environments. Particularly, we utilize multiple robot's activeness and collaborative capability to gather more information efficiently, enhancing the synergy between \textit{sensing} and \textit{scheduling} abilities and further simplifying the perception problem (\ie, GSL). 



% However, realizing the idea is non-trivial and faces grand challenges.
% In reality, the gas landscape is characterized by a \textit{patchy} structure. As demonstrated by field measurements of gas concentration (see (\cref{fig:conc_distr_characteristic})), the gas plumes in realistic atmospheric environments fragment into disjointed patches and form distinct and scattered areas. 
% From the perspective of source seeking robots, the concentration measured along the horizontal centerline exhibits pronounced fluctuations as the distance to the source increases, since gas patches are separated by regions where gas concentration is below detection. 
% This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches and fail to complete GSL.



% \begin{figure}[!t]
%     \setlength{\abovecaptionskip}{0.2cm}
%     \setlength{\belowcaptionskip}{-0.1cm}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figs/fig2.png}
%     \caption{Spatial characteristics of the gas concentration distribution.}
%     \label{fig:conc_distr_characteristic}
% \end{figure}
\begin{figure}[!t]
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/fig2-20240314-220ppi.png}
    % \caption{Real-world spatial characteristics of gas concentration distribution are observed within a sub-area of our testbed. A gas emission device is positioned on the left side, and winds blow from left to right. The heatmap illustrates concentration values, representing the number of particles with a diameter $>$0.3um in 0.1L of air. The gas plume patches may mislead source seeking robots into incorrectly identifying these (false positives) as the actual source of the gas emission. }
    \caption{\rev{\textbf{Spatial characteristics of gas concentration}. We conducted a proof-of-concept experiment to check gas characteristics in our indoor testbed, with a gas emission device at $(1.0,1.0)$ and winds blowing along the $x$ axis. The heatmap illustrates concentration values, representing the number of particles with a diameter $>$0.3um in 0.1L of air. The observed gas plume patches may mislead source-seeking robots into falsely identifying them as the actual gas emission source.}} 
    \label{fig:conc_distr_characteristic}
\end{figure}




% To tackle the above challenge, we propose \textit{GasHunter}, a collaborative robotic olfactory system towards practical gas source localization. The design and implementation of \textit{GasHunter} boosts adaptability to patchiness at both the individual and the team level, making \textit{GasHunter} achieve more efficient and effective emission source localization. For each individual, we devise individual active sensing algorithms aimed at improving the quality of estimation; for the whole team, we develop collaborative roles adaptation strategies to enhance the efficiency of source seeking. Overall, our method features the following two key designs: 

To tackle the aforementioned challenge, we design and implement \textit{GasHunter}, a collaborative olfactory robot scheduling system for gas source localization. Benefiting from \textit{GasHunter}, a team of olfactory robots can dynamically adapt to patchy environmental conditions and adjust their moving trajectories accordingly, enabling efficient and effective emission source localization. In general, \textit{GasHunter} excels in the following two aspects.

% % To achieve individual-level resiliency, we propose a \textit{Patchiness-aware Active Sensing} method. It improves the collected data effectiveness (the quality of sampled data) by movement coordination. This is achieved by adjusting the robots' gradient-based moving direction with a regulation term. This term injects the motion with an appropriate amount of perturbation, enabling them to escape from false positive source positions efficiently.
% \noindent $\bullet$ At the individual level, we propose a \textit{Patchiness-aware Active Sensing} method, which builds on probabilistic source estimation and embeds principles of Langevin MCMC, to improve the quality of collected data and estimation. % (integrates deterministic and stochastic components of sensing direction)
% This is achieved by incorporating a regulatory term into the robots' gradient-based sensing direction. This enables escape from false positive source positions, resulting in the collection of more valid and informative data.

\noindent $\bullet$ \textbf{At the individual level}, we propose a \textit{Patchiness-aware active sensing} method, which refines the probabilistic source estimation by incorporating the patchy characteristic of gas in each robot's moving strategy. Inspired by the principles of Langevin MCMC \cite{deng2020contourSGLD}, we adjust robots' gradient-based moving direction with a regulation term, allowing them to escape false positive source positions and thereby collect more informative sensing data.




% % To implement a system with team-level resiliency, we devise a \textit{Potential-instructed Collaborative Roles Adaptation} strategy for multiple robots. It enhances source-seeking efficiency and accelerate the GSL process. 
% \noindent $\bullet$ At the team level, we devise a \textit{Potential-instructed Collaborative Roles Adaptation} strategy, which leverages both external environmental cues and internal team dynamics, to enhance source-seeking efficiency and accelerate the GSL process. 
% Specifically, robots in the team collaboratively estimate the potential of each position locating the emission source. 
% Those positioned in areas with higher probabilities conduct fine-grained search to inspect spurious concentration maxima (exploiter), while other robots perform coarse-grained search to discover new potential sources (explorer). 
% When an explorer finds potential sources with higher probability than an exploiter, they exchange their roles to allow flexible collaboration. %, so that the explorer becomes an exploiter while the exploiter is released for course-grained search. 
% % In this manner, the robots' roles are adjusted adaptively based on their current positions and the potential to localize the source in the surroundings, thus parallelizing the exploration of the environment and exploitation of collected information in a flexible manner.

\noindent $\bullet$ \textbf{At the team level}, we design a \textit{Potential-instructed collaborative roles adaptation} strategy that further enhances the source-seeking efficiency based on the relationship between the \rev{robots' spatial distribution} and their measurements.  Each robot in the team adopts either a fine-grained search role to inspect spurious signals (\ie, exploiter) or a coarse-grained search role to discover potential new sources (\ie, explorer). These roles are adaptively adjusted based on the estimated probabilities of each robot's proximity to the emission source, thereby parallelizing the exploration of the environment and exploitation of collected information in a flexible manner.




% % To the best of our knowledge, we are the first to handle the turbulent airflow and patchy gas plume issue from the view of nonconvex learning. 
% We validate our design with experiments on a multi-robot testbed in a $15m \times 10m$ space and large scale physical feature based simulations in two different scenarios. Experiment results show that our system achieves a $20\%+$ success rate improvement and a $30\%+$ path efficiency improvement compared to state-of-the-art methods~\cite{reddy2022olfactory,ojeda2021information,vergassola2007infotaxis}.
% % We implemented the proposed system on an indoor gas emission testbed, in a  $15m \times 10m$ space. We build a team of olfactory unmanned ground vehicles to conduct the gas source localization task. 
% % We further conduct comprehensive simulation experiments with various number of robots in two different scenarios (an empty space and a structured environment). 
% % We compare our system with the state-of-the-art (SOTA) of both bio-inspired and probabilistic GSL algorithms, Surge-Cast \cite{reddy2022olfactory} and Infotaxis \cite{ojeda2021information,vergassola2007infotaxis}. The experiment results show that our system achieves success rates higher than baselines by $> 20\%$, outperforming then in path efficiency by $> 32.84\%$. 
% % We then examine the robustness of our system under various conditions and finally conduct an ablations study to understand each module in our system. 



We evaluate the performance of \textit{GasHunter} and compare it with state-of-the-art baseline methods through experiments on a real-time multi-robot testbed and extensive physical feature-based simulations. Experiment results show that our system outperforms all baselines, achieving a $20\%+$ success rate and $30\%+$ path efficiency improvement~\cite{reddy2022olfactory,ojeda2021information,vergassola2007infotaxis}.


We summarize the contributions of this paper as follows:
\begin{itemize}
\item We design \textit{GasHunter}, a collaborative multi-robot olfactory sensing system for gas source localization, specifically designed to handle the patchy characteristic in realistic gas plume environments.
\item We devise a patchiness-aware active sensing method, which builds on probability source estimation and embeds principles of Langevin dynamics, to improve the quality of collected data and estimation.
\item We develop a potential-instructed collaborative roles adaptation strategy, which leverages both external environmental cues and internal team dynamics, to enhance source-seeking efficiency and accelerate the GSL process. 
\item Extensive experiments are conducted for validation and evaluation in both a real-world testbed and a physical-feature-based gas dispersion simulator. 
\end{itemize}

The remainder of the paper is organized as follows. We first introduce the background, motivation, and related works in \cref{sec:background}. In \cref{sec:systemmodel}, we present the overview and components of our system model, followed by problem formulation. In \cref{sec:algo1,sec:algo2}, we introduce the algorithm design, involving detailed descriptions of the patchiness-aware active sensing and potential-instructed collaborative roles adaptation. \cref{sec:eval} showcases the implementation and evaluation. Finally, \cref{sec:conclusion} concludes the paper. 

==> introduction.tex <==
\section{Introduction}


% Accidental or unanticipated gas leaks can create a highly flammable environment, pose health risks, or cause environmental destruction. 
% The Bhopal gas tragedy exposed over 500,000 people to methyl isocyanate (MIC) \cite{mishra2009bhopal}. 
% In the San Juanico incident, a 11,000 $m^3$ LPG leak led to a series of explosions \cite{arturson1987tragedy}. 
% The Aliso Canyon blowout released over 100,000 tonnes of greenhouse gas methane into the atmosphere \cite{conley2016methane}. 
% % Therefore, localize the gas source as soon as possible is crucial for mitigating the severe consequences associated with such incidents (e.g., shutting off gas supply lines or containing leaks). 
% Therefore, localize the gas source as soon as possible is crucial for the following mitigation operations (e.g., shutting off gas supply lines or containing leak). 

\IEEEPARstart{U}{nforeseen} gas leaks can swiftly create a highly flammable atmosphere, which will lead to risks of explosions, health hazards, as well as long-term environmental impacts, especially when the gas is toxic \cite{liu2017individualized, pal2018vehicle, maag2018w}. 
For instance, the Bhopal gas tragedy exposed over 500,000 people to methyl isocyanate (MIC) \cite{mishra2009bhopal}, while the Aliso Canyon blowout released over 100,000 tonnes of greenhouse gas methane into the atmosphere \cite{conley2016methane}. 
Hence, localizing the gas source as soon as possible remains paramount to executing subsequent mitigation measures, such as shutting off valves and effectively containing or sealing the leaks \cite{liu2017delay}.

% However, \textbf{gas source localization (GSL)} is challenging. Long and intricate pipelines present a multitude of potential leakage sources, making it infeasible to position sensors along every inch of the line. Moreover, dispatching human operators to undertake such tedious and dangerous tasks not only puts them in harm's way but is also susceptible to human interpretation error \cite{arain2021sniffing}. 
Nonetheless, \textbf{gas source localization (GSL)} in emergent scenarios poses significant challenges \cite{motlagh2023unmanned, abughanam2023localization}. 
Specifically, extensive and complex pipelines offer numerous potential points of leakage, rendering it impractical to install sensors at every juncture \cite{ojeda2020evaluation}. 
Furthermore, assigning human operators to engage in these laborious and perilous activities not only introduces the risk of human error in interpretation \cite{arain2021sniffing}, but also poses a risk to their health and lives \cite{ojeda2023robotic}.

\begin{figure}[t]
    % \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    % \includegraphics[width=0.6\columnwidth]{figs/scenario.jpeg}
    % \includegraphics[width=0.3\columnwidth]{figs/Qheatmap.png}
    \includegraphics[width=0.98\columnwidth]{figs/fig1.png}
    
    \caption{Mobile olfactory robots autonomously search for and navigate towards the source of gas leakage. }
    \label{fig:scenario}
\end{figure}

% As an alternative, the deployment of autonomous mobile olfactory robots offers a viable solution for gas source localization. This approach is attractive not only for its safety but also its efficiency \cite{arain2021sniffing}. As illustrated in \cref{fig:scenario}, in the event of a gas leakage within a factory's pipeline system, a fleet of robots equipped with gas concentration sensors can be dispatched to search for and locate the source of the leakage. 

Therefore, deploying autonomous mobile olfactory robots for GSL presents a solution with great potential \cite{iyer2019living, moradi2018skycore, khochare2021heuristic}, as they can search the environment with high efficiency without risking human lives \cite{xu2022swarmmap, zhou2022swarm}. 
We task gas leakage in a factory with intricate pipelines as an example as shown in \cref{fig:scenario}. Here, a fleet of robots equipped with gas concentration sensors and wind sensors are dispatched to search the surroundings and gather gas sensory data. By analyzing and interpreting the environmental conditions, the robots autonomously navigate to pinpoint the source of the gas leak.
% This is nontrivial for two reasons. 
% First, as illustrated in \cref{fig:conc_distr_characteristic}, the turbulent airflow in real-world scenarios \cite{kadakia2022odour} causes the gas plume to fragment and become significantly patchy \cite{reddy2022olfactory}. Second, the mobile robots can only access to noisy sensory measurements and partial observations, unable to get an accurate and global understanding of the field. 
% Consequently, inferring the source position from robots' measurements becomes intractable \cite{ojeda2023robotic}. 

% Unfortunately, current approaches are not able to offer feasible solutions for autonomous mobile robot olfaction-based gas source localization in realistic environments, which typically resort to two broad categories of strategies:
Unfortunately, existing approaches are not able to offer feasible GSL solutions for mobile olfaction-based robots in realistic environments. Strategies of GSL can be roughly grouped into two categories:

\begin{figure*}[!t]
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \includegraphics[width=2.0\columnwidth]{figs/fig2.png}
    \caption{Spatial characteristics of the gas concentration distribution.}
    \label{fig:conc_distr_characteristic}
\end{figure*}

\noindent $\bullet$ \textbf{Reactive bio-inspired algorithms}. 
These solutions draw inspiration from the behavior of insects or rodents. They involve moving up the local gas concentration gradients (chemotaxis), responding to air currents and moving upwind (anemotaxis), or combining both \cite{reddy2022olfactory}. 
% However, these reactive methods only works well in continuous concentration fields. In realistic, the gas landscape is discontinuous and patchy (indicating that the gas forms distinct and scattered areas), as shown in \cref{fig:conc_distr_characteristic} (b).
However, these reactive methods only work in ideal continuous concentration fields.
% These reactive methods have been adopted by assuming continuous concentration fields.
Instead, the gas landscape in real-world is usually discontinuous and \textit{patchy} (i.e., the gas forms distinct and scattered areas), as shown in \cref{fig:conc_distr_characteristic}(b).

\noindent $\bullet$ \textbf{Source parameter estimation-based GSL}. 
These solutions estimate the source location utilizing the Bayesian filter, making decisions based on historical data. However, they heavily rely on oversimplified and unrealistic analytical gas plume models, such as the Gaussian plume model\cite{vergassola2007infotaxis, bourne2019CoordinatedBayesianBasedBioinspired, bourne2020decentralized}. These models, as shown in \cref{fig:conc_distr_characteristic} (a), deviate significantly from the complexity of patchy gas distribution in real-world scenarios. 

\IEEEpubidadjcol

\textbf{Our work} aims to deploy and schedule a team of robots to conduct efficient GSL in realistic \textit{patchy} gas environments. 
% Furthermore, we find significant drawbacks when attempting to deploy previous solutions in real-world environments. 
This problem is non-trivial due to the following two challenges:

% Challenge 1: Turbulence, patchy, intermittent
% \noindent $\bullet$ \textbf{The patchy nature of gas plumes confuses and traps robots in gas patches}. 
% Numerous patches create multiple modes (i.e., hills) in the concentration field, causing robots utilizing noisy and local information (e.g., gradient) on such a map to confuse and get stuck in local optima. Additionally, in regions between patches, the robot might have trouble discerning the correct direction to move in due to low or zero gas concentration readings, which make the robot uncertain about whether it is moving towards or away from the source. 
\noindent $\bullet$ \textbf{The patchy nature of gas plumes confuses and traps the robots}. 
% Numerous patches create multiple modes (i.e., hills) in the concentration field, causing robots utilizing noisy and local information (e.g., gradient) on such a map to confuse and get stuck in local optima. Additionally, in regions between patches, the robot might have trouble discerning the correct direction to move in due to low or zero gas concentration readings, which make the robot uncertain about whether it is moving towards or away from the source. 
As demonstrated by experimental data in Fig. \ref{fig:conc_distr_characteristic}(b), plumes fragment into disjointed patches spatially. The gas concentration measured along the horizontal centerline (\cref{fig:conc_distr_characteristic}(c)) exhibits pronounced fluctuations as the distance to the source increases, which indicates the patches are separated by regions where gas concentration is below detection. This intermittent characteristic introduces uncertainty in the source direction when robots devise paths using noisy and local sensory data, ultimately leading to their entrapment within these patches.

% Challenge 2
\noindent $\bullet$ \textbf{Trade-off between source localization effectiveness and search efficiency for collaborative robots}. 
% The robot team conducting GSL strives to i) quickly tell apart spurious gas patches and ii) identify new potential positions of being the gas source. However, it's challenging to make the group behave in a way that does both things well. For example, for the former goal, the team members should gather towards one place, concentrating their efforts and getting more measurements to enhance the accuracy of estimated gas source probability of that place; for the latter, they should scatter and explore disjoint areas independently. 
The robot team conducting GSL strives to (i) identify new potential gas source positions and (ii) exclude false potential source positions. These two goals are inconsistent and render it hard to schedule multiple robots collaboratively. Specifically, for the former goal, the robots are required to disperse and explore disjoint areas independently. Conversely, the latter goal demands the robots to converge to the same location to confirm source probability through multiple measurements.

% In previous works, the following research gaps exist: 
% (1) Escaping from spurious gas patches in turbulent airflow. Previous works either do not explicitly consider the airflow turbulence \cite{reddy2022olfactory}, or rely on oversimplified hence unrealistic gas plume models (e.g., Gauss plume) \cite{vergassola2007infotaxis, bourne2019CoordinatedBayesianBasedBioinspired, bourne2020decentralized}, both ignoring that gas plumes are patchy. Though \cite{ojeda2023robotic} adopts a relatively practical dispersion model, it relies on predictions of unvisited locations' measurements, which are inaccurate.
% (2) Striking a balance between the search accuracy and efficiency via collaboration in a principled way. Existing methods tailored for cooperative GSL either rely on gathering or scattering, so they lack efficiency in achieving both goals. In Particle Swarm Optimization (PSO)-based algorithms \cite{duisterhof2021sniffy}, robots follow the one who discovers a better pattern (potential source), resulting in gathering behavior \cite{chen2019odor}. In contrast, another approach \cite{bourne2019CoordinatedBayesianBasedBioinspired} dispatches robots to investigate several likely source positions separately, inducing scattering behavior. 

In this paper, we propose \textit{GasHunter}, a collaborative multi-robot olfaction-based system for gas source localization. \textit{GasHunter} features two key designs from non-convex learning perspective to conquer the patchy characteristic of gas plumes and enable efficient and effective source localization by a collaborative strategy, as elaborated below.

% To address the first challenge, we design a novel \textit{patchy plume-resilient movement planning} algorithm for GSL, borrowing ideas from nonconvex learning and driving the robot's motion by Langevin diffusion. In this manner, we empower the robot to escape from spurious local minima, navigate across patchy gas plumes efficiently, and reach the source of gas leakage within a shorter time. 

To address the first challenge, we propose a novel \textit{Patchy Plume-Resilient Movement Planning} method, borrowing ideas from Langevin diffusion in non-convex learning to drive the robot's moving direction. Unlike current practices where robots move based on reactive stimulus or oversimplified and unrealistic analytical gas plume models, this method adjusts the robots' moving direction with a regulation term, enabling them to escape from false positive source positions efficiently.

% a tightly-collaborated and systematically-coordinated multi-robot GSL algorithm
% To address the second challenge, we propose a tightly-collaborated and systematically-coordinated multi-robot GSL strategy \textit{CoRA}, \textbf{Co}llaborative team \textbf{R}oles \textbf{A}daptation, balancing the search efficiency and localization accuracy by performing exploitation parsimoniously and executing exploration appropriately. The \textit{CoRA} module involves two components. First, robots in a team are assigned heterogeneous roles. Some are responsible for distinguishing spurious concentration maxima (\textit{exploiter}), others are in charge of discovering new potential source positions (\textit{explorer}). Second, team roles are adjusted adaptively. If an exploiter is situated at the position with higher probability of locating the source than an explorer, the two robots exchange their roles. 
% In contrast, existing methods tailored for cooperative GSL either rely on gathering or scattering, so they lack efficiency in achieving both goals. In Particle Swarm Optimization (PSO)-based algorithms \cite{duisterhof2021sniffy}, robots follow the one who discovers a better pattern (potential source), resulting in gathering behavior \cite{chen2019odor}. On the contrary, another approach \cite{bourne2019CoordinatedBayesianBasedBioinspired} dispatches robots to investigate several likely source positions separately, inducing scattering behavior. 


To address the second challenge, we devise a \textit{Collaborative Roles Adaptation} strategy for multiple robots to balance the search efficiency and localization effectiveness. Robots are assigned heterogeneous roles that represent different planning preferences. For example, some robots are responsible for inspecting spurious concentration maxima (\textit{exploiter}), while others are in charge of discovering new potential source positions (\textit{explorer}). The robots' roles are adjusted adaptively based on their current positions and the potential to localize the source in the surroundings, thus parallelizing the exploration of the environment and exploitation of collected information in a flexible manner.

% In contrast, existing methods tailored for cooperative GSL either rely on gathering or scattering, so they lack efficiency in achieving both goals. In Particle Swarm Optimization (PSO)-based algorithms \cite{duisterhof2021sniffy}, robots follow the one who discovers a better pattern (potential source), resulting in gathering behavior \cite{chen2019odor}. On the contrary, another approach \cite{bourne2019CoordinatedBayesianBasedBioinspired} dispatches robots to investigate several likely source positions separately, inducing scattering behavior. 

% To the best of our knowledge, we are the first to handle the turbulent airflow and patchy gas plume issue from the view of nonconvex learning. 
We validate our design with experiments on a multi-robot testbed in a $15m \times 10m$ space and large scale physical feature based simulations in two different scenarios. Experiment results show that our system achieves $20\%+$ success rate improvement and $30\%+$ path efficiency improvement compared to state-of-the-art methods~\cite{reddy2022olfactory,ojeda2021information,vergassola2007infotaxis}.
% We implemented the proposed system on an indoor gas emission testbed, in a  $15m \times 10m$ space. We build a team of olfactory unmanned ground vehicles to conduct the gas source localization task. 
% We further conduct comprehensive simulation experiments with various number of robots in two different scenarios (an empty space and a structured environment). 
% We compare our system with the state-of-the-art (SOTA) of both bio-inspired and probabilistic GSL algorithms, Surge-Cast \cite{reddy2022olfactory} and Infotaxis \cite{ojeda2021information,vergassola2007infotaxis}. The experiment results show that our system achieves success rates higher than baselines by $> 20\%$, outperforming then in path efficiency by $> 32.84\%$. 
% We then examine the robustness of our system under various conditions and finally conduct an ablations study to understand each module in our system. 
We summarize the contributions of this paper as follows:
% \begin{itemize}
% \item A patchy plume-resilient movement strategy that navigates across patchy gas plumes. 
% \item A heterogeneous team roles assignment and adaptation algorithm that balances search efficiency (global exploration) and localization effectiveness (local exploitation) by role-swapping, incorporating replica exchange. 
% \item Validation and evaluation in both a testbed and a physical-feature-based gas dispersion simulator rooted in the principles of Computational Fluid Dynamics. 
% \end{itemize}
\begin{itemize}[topsep=3pt, partopsep=2pt]
\item We design \textit{GasHunter}, a collaborative multi-robot olfactory sensing system for gas source localization, specifically designed to handle the patchy characteristic in realistic gas plume environments.
\item We devise a patchy plume-resilient movement strategy inspired by non-convex learning to conquer the complex patchy characteristic of gas plumes.
\item We develop a collaborative strategy for multiple robots by assigning and adapting their planning preferences dynamically to balance the search efficiency and localization effectiveness of gas sources.
\item Extensive experiments are conducted for validation and evaluation in both a real-world testbed and a physical-feature-based gas dispersion simulator. 
\end{itemize}

The remainder of the paper is organized as follows. We first introduce the background, motivation, and related works in \cref{sec:background}. In \cref{sec:systemmodel}, we present the overview and components of our system model, followed by problem formulation. In \cref{sec:algo1,sec:algo2}, we introduce the algorithm design, involving detailed descriptions of the patchy plume-resilient movement planning and collaborative roles adaptation. \cref{sec:eval} showcases the implementation and evaluation. Finally, \cref{sec:conclusion} concludes the paper. 
